Dynamical supersymmetry enhancement of black hole horizons

This thesis is devoted to the study of dynamical symmetry enhancement of black hole horizons in string theory. In particular, we consider supersymmetric horizons in the low energy limit of string theory known as supergravity and we prove the $\textit{horizon conjecture}$ for a number of supergravity theories. We first give important examples of symmetry enhancement in $D=4$ and the mathematical preliminaries required for the analysis. Type IIA supergravity is the low energy limit of $D=10$ IIA string theory, but also the dimensional reduction of $D=11$ supergravity which itself the low energy limit of M-theory. We prove that Killing horizons in IIA supergravity with compact spatial sections preserve an even number of supersymmetries. By analyzing the global properties of the Killing spinors, we prove that the near-horizon geometries undergo a supersymmetry enhancement. This follows from a set of generalized Lichnerowicz-type theorems we establish, together with an index theory argument. We also show that the symmetry algebra of horizons with non-trivial fluxes includes an $\mathfrak{sl}(2, \mathbb{R})$ subalgebra. As an intermediate step in the proof, we also demonstrate new Lichnerowicz type theorems for spin bundle connections whose holonomy is contained in a general linear group. We prove the same result for Roman's Massive IIA supergravity. We also consider the near-horizon geometry of supersymmetric extremal black holes in un-gauged and gauged 5-dimensional supergravity, coupled to abelian vector multiplets. We consider important examples in $D=5$ such as the BMPV and supersymmetric black ring solution, and investigate the near-horizon geometry to show the enhancement of the symmetry algebra of the Killing vectors. We repeat a similar analysis as above to prove the horizon conjecture. We also investigate the conditions on the geometry of the spatial horizon section $\cal{S}$.

==> dedication/dedication.tex <==
\cleardoublepage

\begin{dedication}
  Dedication here.
\end{dedication}

==> introduction/introduction_-_Copy.tex <==
\chapter{Introduction}
\section{Black holes}
A black hole is a region of spacetime that has such strong gravitational effects that nothing, not even light can escape. This literally makes the region black as no photons or massive particles are able to escape this region, and hence we cannot observe it. In other words, it is the region where light rays cannot escape to infinity. They can be formed from the gravitational collapse of massive stars but are also of interest in their own right, independently of how they were formed. Far from being hungry beasts devouring everything in their vicinity as shown in popular culture, we now believe certain (supermassive) black holes actually drive the evolution of galaxies \cite{richstone}.

In 2016, the Laser Interferometer Gravitational-Wave Observatory (LIGO) made the first detection of gravitational waves from a binary black hole merger \cite{abbott} which was a milestone in physics and astronomy. It confirmed a major prediction of Einstein's general theory of relativity and marked the beginning of the new field of gravitational-wave astronomy. Gravitational waves carry information about their origins and about the nature of gravity that cannot otherwise be obtained. The gravitational waves were produced in the final moments before the merger of two black holes, 14 and 8 times the mass of the sun to produce a single black hole 21 times the mass of the sun. During the merger, which occurred approximately 1.4 billion years ago, a quantity of energy roughly equivalent to the mass of the sun was converted into gravitational waves. The detected signal comes from the last 27 orbits of the black holes before their merger. In 2017, another observation by LIGO and Virgo gravitational-wave detectors of a binary neutron star inspiral signal, called GW170817 \cite{ligo1} and associated to the event a gamma ray burst \cite{ligo2} was independently observed \cite{ligo3}. These led to new bounds and constraints for fundamental physics, such as the stringent constraint on the difference between the speed of gravity and the speed of light, a new bound on local Lorentz invariance violations and a constraint on the Shapiro delay between gravitational and electromagnetic radiation which enabled a new test of the equivalence principle \cite{ligo2}. As a result, these bounds also constrain the allowed parameter space of the alternative theories of gravity that offer gravitational explanations for the origin of dark energy or dark matter.

Black hole research is at the forefront of modern physics because much about black holes is still unknown. Currently, the best two theories we have that describe the known universe are the Standard model of particle physics (a quantum field theory) and general relativity (a classical field theory). Most of the time these two theories do not talk to each other, with the exception of two arenas: the singularity before the Big Bang and the singularity formed within a black hole. The singularity is a point of infinite density and thus the physical description necessarily requires quantum gravity. Indeed Roger Penrose and Stephen Hawking also showed 48 years ago that, according to general relativity, any object that collapses to form a black hole will go on to collapse to a singularity inside the black hole \cite{penrose}. This means that there are strong gravitational effects on arbitrarily short distance scales inside a black hole and such short distance scales, we certainly need to use a quantum theory to describe the collapsing matter.  

General relativity is not capable of describing what happens near a singularity and if one tries to quantize gravity \textit{naively}, we find divergences that we can't cancel because gravity is non-renormalizable.\footnote{In particular, the number of counterterms in the Lagrangian, required to cancel the divergences is infinite and thus the process of renormalization fails.} 
String theory is a broad and varied subject that attempts to remedy this and to address a number of deep questions of fundamental physics. It has been applied to a variety of problems in black hole physics, early universe cosmology, nuclear physics, and condensed matter physics, and it has stimulated a number of major developments in pure mathematics. Because string theory potentially provides a unified description of gravity and particle physics, it is a candidate for a theory of everything, a self-contained mathematical model that describes all fundamental forces and forms of matter.

\begin{comment}
In 1964, Roger Penrose proves that an imploding star will necessarily produce a singularity once it has formed an event horizon. The presence of a singularity in the classical thoery also means that once we go sufficiently far into the black hole, we can no longer predict what will happen. It is hoped that this failure of the classical theory can be cured by quantizing gravity as well.
\end{comment}

In the currently accepted models of stellar evolution, black holes are thought to arise when massive stars undergo gravitational collapse, and many galaxies are thought to contain supermassive black holes at their centers. Black holes are also important for theoretical reasons, as they present profound challenges for theorists attempting to understand the quantum aspects of gravity. String theory has proved to be an important tool for investigating the theoretical properties of black holes because it provides a framework in which theorists can study their thermodynamics, aided in particular by properties such as supersymmetry.

When we talk about the masses of black holes, we usually compare them with the mass of our Sun (also known as a solar mass denoted by $M_{\odot}$). Based upon the length of the year, the distance from Earth to the Sun (an astronomical unit or AU), and the gravitational constant (G), one solar mass is given by:
\bea
M_{\odot}={\frac {4\pi ^{2}\times (1\,\mathrm {AU} )^{3}}{G\times (1\,\mathrm {yr} )^{2}}} = (1.98855 \pm 0.00025) \times 10^{30} kg \ .
\ee
There are three types of black holes that can arise:
\begin{itemize}
\item Stellar black holes are formed from the gravitational collapse of a massive star. They have masses ranging from about 5-99$M_{\odot}$
\item Supermassive black holes are the largest type, on the order of $10^2-10^{12} M_{\odot}$
\item Miniature black holes, also known as quantum mechanical black holes are a hypothetical tiny black holes, for which quantum mechanical effects play a role. These will have masses about the same as Mount Everest.
\end{itemize}

The first person to come up with the idea of a black hole was John Mitchell in 1783,
followed (independently) by Pierre-Simon Laplace in 1796. These prototypical black objects, called 'dark stars', were considered from the point of view of Newtons law of motion and gravitation. In particular Mitchell calculated that when the escape velocity at the surface of a star was equal to or greater than lightspeed, the generated light would be gravitationally trapped, so that the star would not be visible to a distant astronomer.  The event horizon is the boundary of this region, also known as the `point of no return', because once you go past this point it is impossible to turn back. To see this, consider an object of mass $m$ and a spherically symmetric body of mass $M$ and radius $R$. The total energy is,
\begin{eqnarray}
\label{te}
E = \frac{1}{2}m v^2 - \frac{G m M}{r} \ ,
\end{eqnarray}
where $r$ is the distance from the centre of mass of the body to the object. We can also write this as $r = R + h$, where $h$ is the distance from the surface of the body to the object, but the region we will consider is at $r \geq R$ or $h \geq 0$. An object that makes it to $r \rightarrow \infty$ will have $E \geq 0$ as the kinetic energy will dominate for large $r$. This implies,
\begin{eqnarray}
v \geq v_e(r) \equiv \sqrt{\frac{2GM}{r}} \ ,
\end{eqnarray}
where $v_e(r)$ is the escape velocity, which is the lowest velocity which an object must have in order to escape the gravitational attraction from a spherical body of mass $M$ at a given distance $r$. By energy conservation, we have at the surface of the body ($r=R$),
\begin{eqnarray}
v \geq  v_{e}(R) = \sqrt{\frac{2GM}{R}} \ .
\end{eqnarray}
This is independent of the the mass of the escaping object, by the equivalence of inertial and gravitational masses. Now the escape velocity at the surface is greater than the speed of light, $v_e (R) > c$ if
\begin{eqnarray}
R < r_s \equiv \frac{2GM}{c^2} \ .
\end{eqnarray}
The radius $r_s$ is now understood in terms of the Schwarzschild radius. The surface $r = r_s $ acts as an ``event horizon" if the body fits inside this radius. Of course, there is nothing particularly special about the speed of light $c$ in the Newtonian (non-relativistic) gravity. Objects in principle could move faster than $c$ which means that they may always escape the would-be black hole. Moreover,
a photon emitted from such an object does leave the object, although it would eventually fall back in. Thus there are no real black holes (a body from which nothing can escape) in Newton's gravity. 

As we now understand photons to be massless, so the naive
analysis described above is not physically realistic.
However, it is still interesting to consider such objects as a starting point.
The consideration of such ``dark stars" raised the intriguing possibility that
the universe may contain a large number of massive objects which cannot be
observed directly. This principle turns out to be remarkably close to our current understanding of cosmology. However, the accurate description of a black hole has to be general relativistic.
\begin{figure}[h!]
\begin{center}
	\includegraphics[width=200pt]{sradius.png}
\end{center}
	\caption{Event horizon of a black hole enclosing a singularity (credit: \url{https://goo.gl/CAXqfD})}
	\label{fig:sradius}
\end{figure}
Isaac Newton was to be overturned by Albert Einstein with his special theory of relativity in 1905, which showed that the speed of light was constant in any reference frame and then his general theory of relativity in 1915 which describes gravity as the curvature of space-time \cite{einsteingr};
\bea
R_{\mu \nu} - \frac{1}{2}R g_{\mu \nu} = 8 \pi G T_{\mu \nu} \ .
\ee
The theory relates the metric tensor $g_{\mu \nu}$, which defines a spacetime geometry, with a source of gravity that is associated with mass or energy and $R_{\mu \nu}$ is the Ricci tensor.
Black holes arise in general relativity as a consequence of the solution 
to the Einstein field equations found by  Karl Schwarzschild in 1916.
Although the Schwarzschild solution was originally formulated in order
to describe the gravitational field of the solar system, and to
understand the motion of objects passing through this field, 
the idea of a black hole remained as an intriguing possibility.
Einstein himself thought that these solutions were simply a mathematical curiosity and not physically relevant. In fact, in 1939 Einstein tried to show that stars cannot collapse under gravity by assuming matter cannot be compressed beyond a certain point. 

The Schwarzschild radius can also be realized by considering the Schwarzschild solution in general relativity i.e any non-rotating, non-charged spherically-symmetric body that is smaller than its Schwarzschild radius forms a black hole. This idea was first promoted by David Finkelstein in 1958 who theorised that the Schwarzschild radius of a black holes is a causality barrier: an event horizon. The Schwarzschild solution is an exact solution and  was found within only a few months of the publication of Einstein’s field equations. Instead of dealing only with small weak-field corrections to Newtonian gravity, fully nonlinear features of the theory could be studied, most notably gravitational collapse and singularity formation. The Schwarzschild metric written in Schwarzschild Coordinates $(t, r, \theta, \varphi)$ is given by,
\bea
ds^2 = -f(r) c^2 dt^2 + f(r)^{-1} dr^2 + r^2 \left(d\theta^2 + \sin^2\theta \, d\varphi^2\right) \ ,
\ee
where $f(r) = 1-r_s / r$. In this form, the metric has a coordinate singularity at $r=r_s$ which is removable upon an appropriate change of coordinates. The Kretschmann scalar for this metric elucidates the fact that the singularity at $r=0$ cannot be removed by a coordinate transformation,
\bea
R_{\mu \nu, \rho \sigma}R^{\mu \nu, \rho \sigma} = \frac{4G^2M^2}{c^4 r^6} \ ,
\ee
where $R_{\mu \nu, \rho \sigma}$ is the Riemann tensor. A more accurate general relativistic description of the event horizon is that within this horizon all light-like paths and hence all paths in the forward light cones of particles within the horizon are warped as to fall farther into the hole.

\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=200pt]{tipping.jpg}
	\end{center}
  \caption{Light cones tipping near a black hole (credit: \url{https://goo.gl/riTdG1})}
  \label{fig:tipping}
\end{figure}

In order to define the black hole region and event horizon in a concrete way, we will need to consider some definitions. Let $({\cal M},g)$ be an asymptotically flat manifold.
\theoremstyle{definition}
\begin{definition}{The {\bf causal past} of $U \subset {\cal M}$ is}
\begin{eqnarray}
\label{cp}
J^{-}(U) = \big\{p\in {\cal M} : \exists \textrm{a future directed causal curve from }p \textrm{ to some } q\in U \big\} \nonumber \ .
\end{eqnarray}\end{definition}Let us denote $\mathscr{I}^+$ as {\bf future null infinity}, the limit points of future directed null rays in ${\cal M}$.
\theoremstyle{definition}
\begin{definition}{The {\bf black hole region} $B$ is the region of spacetime in ${\cal M}$ that is not contained in the Causal past of future null infinity $J^{-}(\mathscr{I}^+)$, $B = {\cal M} \setminus J^{-}(\mathscr{I}^+)$ i.e}
\begin{eqnarray}
\label{bhr}
B &=& \big\{p\in {\cal M} : \exists \textrm{ no future directed casual curve from }p\textrm{ to }\mathscr{I}^+ \big\} \nonumber \ .
\end{eqnarray}
\end{definition}
\theoremstyle{definition}
\begin{definition}{The {\bf event horizon} $\cal{H}$ is the boundary of $B$ in ${\cal M}$ i.e the boundary of the causal past of future null infinity $J^{-}(\mathscr{I}^+)$ in ${\cal M}$, ${\cal{H}} = \partial B = \partial J^{-}(\mathscr{I}^+)$}
\end{definition}
\begin{figure}[h!]
	\begin{center}
	\includegraphics[width=180pt]{penrose.jpg}	
	\end{center}
  \caption{Penrose diagram of a collapsing star where $i^+$, $i^-$ denote future and past timelike infinity respectively and $i^0$ is spacelike infinity}
  \label{fig:penrose}
\end{figure}
\theoremstyle{definition}
\begin{definition}{A hypersurface $\cal{H}$ defined by a smooth function $S(x^{\mu}) = 0$, where $S \in  C^{\infty}({\cal M})$ is called a {\bf null hypersurface} if the normal vector field $\xi^{\mu} \sim g^{\mu \nu}\partial_{\nu}S$ is null, $g(\xi, \xi)=g_{\mu \nu}\xi^{\mu}\xi^{\nu} = 0$ on $\cal{H}$.}
\end{definition}
For such surfaces one can show that
\begin{eqnarray}
\xi^{\nu}\nabla_{\nu}\xi^{\mu} = \kappa \xi^{\mu} \ ,
\end{eqnarray}
where $\kappa$ is a measure to the extent to which the parametrization is not affine. In the context of killing horizons, $\kappa$ can physically be interpreted as the surface gravity, which we will see in the next section. If we denote $l$ to be the normal to $\cal{H}$ which corresponds to an affine parametrization, i.e $l^{\nu}\nabla_{\nu}l^{\mu} = 0$ and $\xi = f(x)l$ for some $f(x)$ then $\kappa = \xi^{\mu}\partial_{\mu}\ln |f|$.

One can also show that the event horizon $\cal{H}$ is a null hypersurface, since all its normals are null on $\cal{H}$. The advantage of the event horizon $\cal{H}$ is that the boundary of a past set is always a null hypersurface and is ruled by null geodesics which stay on the boundary. This is allows one to to prove general properties of the horizon. The disadvantage is that the event horizon cannot be determined locally and one needs the entire future of the spacetime to know where the event horizon is. For practical reasons one might a consider a more local definition of a horizon.


\subsection{Other solutions: Reisser-Nordstr\"om metric (1918)}

The existence of the Schwarzschild solution set in motion a search for other
exact solutions. In 1918, Reissner and Nordstr\"om solved
the Einstein-Maxwell field equations for charged spherically-symmetric non-rotating
systems. Gravity coupled to the electromagnetic field is described by the Einstein-Maxwell action
\bea
S = \frac{1}{16 \pi G} \int \sqrt{-g}(R - F_{\mu \nu}F^{\mu \nu})d^4 x \ ,
\ee
where $F_{\mu \nu} = \nabla_{\mu}A_{\nu} - \nabla_{\nu}A_{\mu}$ and $A_{\mu}$ is the electromagnetic (four-)potential. The normalisation of the Maxwell term is such that the Coulomb force between two charges $Q_1$ and $Q_2$ separated by a sufficiently large distance $r$ is
\bea
F_{Coulomb} = G \frac{|Q_1 Q_2|}{r^2} \ .
\ee
This corresponds to geometrised units of charge.
The equations of motion derived from the variation of the Einstein-Maxwell action are
\bea
R_{\mu \nu} - \frac{1}{2} R g_{\mu \nu} &=& 2\bigg(F_{\mu \lambda}F_{\nu}{}^{\lambda} - \frac{1}{4}g_{\mu \nu}F_{\rho \sigma}F^{\rho \sigma}\bigg) \ ,
\nonumber \\
\nabla_{\mu}F^{\mu \nu} &=& 0 \ .
\ee
They admit the spherically symmetric solution
\bea
ds^2 &=& -\bigg(1 - \frac{2M}{r} + \frac{Q^2}{r^2}\bigg)dt^2 + \bigg(1 - \frac{2M}{r} + \frac{Q^2}{r^2}\bigg)^{-1}dr^2 + r^2 d\Omega^2_2
\cr
&=& -\bigg(1-\frac{r_+}{r}\bigg)\bigg(1-\frac{r_-}{r}\bigg)dt^2 +\bigg(1-\frac{r_+}{r}\bigg)^{-1}\bigg(1-\frac{r_-}{r}\bigg)^{-1}dr^2 + r^2 d\Omega^2_2 \ ,
\nonumber \\
\label{rnsolution}
\ee
which is known as the Reissner-Nordstr\"om solution and the two horizons given by $r_{\pm} = M \pm \sqrt{M^2 -Q^2}$. The extremal limit where the horizons coincide corresponds to $Q=M$. The electric potential is $A_{t} = \frac{Q}{r}$ and the other components of $A_{\mu}$ vanish. We therefore interpret $Q$ as the electric charge of the black hole and $M$ as its mass. Without loss of generality we assume that $Q > 0$. By a theorem analogous to Birkhoff's theorem, the Reissner-Nordstrom solution is the unique spherically symmetric solution to the 
Einstein-Maxwell equations.

Gravitatational theories coupled to Maxwell but also {\it dilaton} fields $\Phi$ emerge from several more fundemental theories such with Kaluza-Klein reduction and compactification. The addition of the dilaton field and the dynamics of the black hole in this theory display interesting properties when compared to the standard Reissner-Nordstr\"om black hole. For this reason, we briefly consider an Einstein-Maxwell gravity coupled to a dilaton field $\Phi$ with dilaton coupling constant $\alpha$. The action is,
\bea
S = \frac{1}{16 \pi G} \int \sqrt{-g}(R -2\nabla^{\mu}\nabla_{\mu}\Phi - e^{-2\alpha \Phi}F_{\mu \nu}F^{\mu \nu})d^4 x \ .
\ee
The equations of motion derived from this variation are
\bea
R_{\mu \nu} - \frac{1}{2} R g_{\mu \nu} &=& 2\bigg(F_{\mu \lambda}F_{\nu}{}^{\lambda} - \frac{1}{4}g_{\mu \nu}F_{\rho \sigma}F^{\rho \sigma}\bigg) + 2\nabla_{\mu} \nabla_{\nu} \Phi - g_{\mu \nu}\nabla^{\lambda}\nabla_{\lambda}\Phi \ ,
\nonumber \\
\nabla_{\mu}(e^{-2\alpha \Phi}F^{\mu \nu}) &=& 0 \ ,
\nonumber \\
\nabla^{\mu}\nabla_{\mu}\Phi &=& \frac{1}{2}\alpha e^{-2\alpha \Phi}F_{\rho \sigma}F^{\rho \sigma} \ .
\ee
The parameter $\alpha$ is a dimensionless constant and the behaviour of the theory shows non-trivial dependence on $\alpha$. The spherically symmetric black hole solutions of this action are given by,
\bea
ds^2 &=& -\bigg(1-\frac{r_+}{r}\bigg)\bigg(1-\frac{r_-}{r}\bigg)^{\frac{1-\alpha^2}{1+ \alpha^2}}dt^2 +\bigg(1-\frac{r_+}{r}\bigg)^{-1}\bigg(1-\frac{r_-}{r}\bigg)^{\frac{\alpha^2 - 1}{1+ \alpha^2}}dr^2 
\nonumber \\
&+& r^2\bigg(1-\frac{r_-}{r}\bigg)^{\frac{2\alpha^2}{1+\alpha^2}} d\Omega^2_2 \ ,
\ee
where the two inner and outer horizons are located at,
\bea
r_+ = M + \sqrt{M^2 - (1-\alpha^2)Q^2},~~ r_{-} = \bigg(\frac{1+\alpha^2}{1-\alpha^2}\bigg)(M - \sqrt{M^2 - (1-\alpha^2)Q^2}) \ .
\nonumber
\ee
The extremal limit where the two horizons coincide corresponds to $Q = M\sqrt{1+\alpha^2}$, and the Maxwell and dilaton fields are
\bea
A_{t} = \frac{Q}{r},~~ e^{2 \alpha \Phi}=
\bigg(1-\frac{r_-}{r}\bigg)^{\frac{2\alpha^2}{1+\alpha^2}} \ .
\ee
For $\alpha < 1$ in order to preserve reality one must have $|\frac{Q}{M}| \leq \frac{1}{\sqrt{1-\alpha^2}}$ but for $\alpha > 1$ we do not have this restriction. 

\subsection{Kerr metric (1963)}
Already in 1918, Lense and Thirring had found the exterior field of a rotating sphere to the first order in the angular momentum, but many were after  a simple exact solution that was physically relevant.
Astrophysically, we know that stars (and for that matter planets) rotate, and from the weak-field approximation to the Einstein equations we even know the approximate form of the metric at sufficiently large distances from a
stationary isolated body of mass $M$ and angular momentum $J$, given by
\bea
ds^2 &=& -\bigg[1 - \frac{2M}{r} + O\bigg(\frac{1}{r^2}\bigg)\bigg]dt^2 
- \bigg[\frac{4 J \sin^2 \theta}{r} + O\bigg(\frac{1}{r^2}\bigg)\bigg]d \phi dt
\nonumber \\
&+& \bigg[1 + \frac{2M}{r} + O\bigg(\frac{1}{r^2}\bigg)\bigg] \bigg(dr^2 + r^2 \left(d\theta^2 + \sin^2\theta \, d\varphi^2\right)\bigg) \ .
\ee
This approximate metric is perfectly adequate for almost all solar system
tests of general relativity, but there certainly are well-known astrophysical
situations (e.g. neutron stars) for which this approximation is inadequate
and so a ``strong field" solution is physically called for. Furthermore,
if a rotating star were to undergo gravitational collapse, then the resulting
black hole would be expected to retain at least some fraction of its initial
angular momentum — thus suggesting on physical grounds that somehow
there should be an extension of the Schwarzschild geometry to the situation
where the central body carries angular momentum.
From the weak-field asymptotic result we can already see that angular
momentum destroys spherical symmetry, and this lack of spherical symmetry
makes the calculations much more difficult. It is not that the basic principles
are all that different, but simply that the algebraic complexity of the computations are much higher.

In 1963, Kerr solved the Einstein vacuum field equations for uncharged symmetric rotating systems, deriving the Kerr metric. It took almost 50 years to find such a solution: the Kerr metric which is a metric that describes the geometry of a spacetime for a rotating black hole with mass $M$ and angular momentum $J$. The Kerr metric describes the geometry of spacetime in the vicinity of a mass $M$ rotating with angular momentum $J$ is
\bea
ds^{2}&=&-\bigg(1-{\frac {r_{s}r}{\Sigma }}\bigg)c^{2}dt^{2}+{\frac {\Sigma }{\Delta }}dr^{2}+\Sigma d\theta ^{2}
\nonumber \\
&+&(r^{2}+a^{2}+{\frac {r_{s}ra^{2}}{\Sigma }}\sin ^{2}\theta )\sin ^{2}\theta \ d\phi ^{2}-{\frac {2r_{s}ra\sin ^{2}\theta }{\Sigma }}\,c\,dt\,d\phi \ ,
\label{kerrsol}
\ee
where the coordinates  $r,\theta ,\phi$  are standard spherical coordinate system, which are equivalent to the cartesian coordinates
\bea
x &=& \sqrt {r^2 + a^2} \sin\theta\cos\phi \ ,
\nonumber \\
y &=& \sqrt {r^2 + a^2} \sin\theta\sin\phi \ ,
\nonumber \\
z &=& r\cos \theta \ ,
\ee
and $r_s$ is the Schwarzschild radius, and where the length-scales $a, \Sigma$ and $\Delta$ have been introduced for brevity,
\bea
a &=&\frac {J}{Mc} \ ,
\nonumber \\
\Sigma &=& r^{2}+a^{2}\cos ^{2}\theta \ ,
\nonumber \\
\Delta &=& r^{2}-r_{s}r+a^{2} \ .
\ee
Astrophysical black holes have a null charge $Q$ and they all
belong to the Kerr family (when $a = 0$ it reduces to the Schwarzschild solution). In contrast to the Kerr solution, the Reissner-Nordstr\"om solution of Einstein's equation is spherically symmetric
which makes the analysis much simpler. Now that another 50 years have elapsed, we can see what an enormous impact this discovery has had. Practically every subfield of general relativity has been influenced. And in astrophysics the discovery of rotating black holes together with a simple way to treat their properties has revolutionized the subject.

\subsection{The Kerr-Newman Geometry (1965)} 

The Kerr-Newmann solution is the most general metric that describes the geometry of spacetime for a rotating charged black hole with mass mass $M$, charge $Q$ and angular momentum $J$. The metric is
\bea
ds^2 =-\bigg({\frac {dr^{2}}{\Delta }}+d\theta ^{2}\bigg)\Sigma+(c\,dt-a\sin ^{2}\theta \,d\phi )^{2}{\frac {\Delta }{\Sigma}} -((r^{2}+a^{2})d\phi -ac\,dt)^{2}{\frac {\sin ^{2}\theta }{\Sigma}} \ ,
\nonumber \\
\label{kerrnewsol}
\ee
where the coordinates $(r, \theta, \phi)$ are standard spherical coordinate system, and the length-scale,
\bea
\Delta &=& r^{2}-r_{s}r+a^{2}+r_{Q}^{2} \ ,
\ee
have been introduced for brevity. Here $r_s$ is the Schwarzschild radius , $G$ is the gravitational constant, and $r_Q$ is a length-scale corresponding to the electric charge $Q$ of the mass
\bea
r^2_{Q} = \frac{Q^2 G}{4\pi \epsilon_0 c^4} \ .
\ee
In this metric, $a=0$ is a special case of the Reissner-Nordstr\"om solution, while $Q=0$ corresponds to the Kerr solution.

\subsection{The No Hair Theorem}
In 1967, Werner Israel \cite{israel1} presented the proof of the no-hair theorem at King's College London. The no-hair theorem postulates that all black hole solutions of the Einstein-Maxwell equations of gravitation and electromagnetism in general relativity can be completely characterized by only three externally observable classical parameters. After the first version of the no-hair theorem for the uniqueness of the Schwarzschild metric in 1967, the result was quickly generalized to the cases of charged or spinning black holes \cite{israel2, carter}. 

In $D=4$ these imply that the Einstein equations admit a unique class of asymptotically flat black hole solutions, parametrized by $(M, Q, J)$. A key step is to establish the horizon topology theorem, which proves that the event horizon of a stationary black hole must have $S^2$ topology \cite{Htopology1}, which was shown in 1972. All other information about the matter which formed a black hole or is falling into it, ``disappears" behind the black-hole event horizon and is therefore permanently inaccessible to external observers. 

\subsubsection{Higher dimensional black holes}

The proof the no-hair theorem relies on the Gauss-Bonnet theorem applied to the 2-manifold spatial horizon section, and therefore does not generalize to higher dimensions. Thus for dimensions $D>4$, uniqueness theorems for asymptotically flat black holes lose
their validity. Indeed, the first example of how the classical uniqueness theorems 
break down in higher dimensions is given by the five-dimensional black ring solution
\cite{Emparan:2001wn, BR1}. There exist black ring solutions with the same asymptotic
conserved charges as BMPV black holes, but with a different horizon topology.  Even more exotic solutions in five dimensions are now known to exist,
such as the solutions obtained in \cite{Horowitz:2017fyg}, describing asymptotically flat black holes which possess a non-trivial topological structure outside the event horizon, but whose
near-horizon geometry is the same as that of the BMPV solution.

The known black hole solutions in four dimensions have been generalised to higher
dimensions. For instance, there exists a solution to the Einstein equations in any dimension $D$,
which is a generalization of the Schwarzschild metric which was discovered by Tangherlini \cite{Tangherlini}. In $d$ dimensions, a Reissner-Nordstr\"om black hole has the metric,
\bea
ds^2 = -\bigg(1-\frac{2\mu}{r^{D-1}} + \frac{q}{r^{2(D-3)}}\bigg)dt^2 + \bigg(1-\frac{2\mu}{r^{d-1}} + \frac{q}{r^{2(D-3)}}\bigg)^{-1}dr^2 + r^2 d\Omega_{D-1}^2 \ ,
\ee
where
\bea
\mu = \frac{8 \pi G M}{(D-2)\Omega_{D-1}},~~ q = \frac{8 \pi G Q^2}{(D-3)(D-2)\Omega_{D-1}},~~ \Omega_{D-1} = \frac{2\pi}{\Gamma(\tfrac{D-1}{2})} \ ,
\ee
and $\Omega_{d-1}$ is the volume of the sphere $S^{d-1}$ and the horizons are located at $r_{\pm} = (\mu \pm \sqrt{\mu^2 - q})^{\tfrac{1}{d-3}}$.
Furthermore, generalisation of the the Kerr metric to higher dimensions was found by Myers and Perry \cite{myers}. The Myers Perry
solution is specified by the mass $M$ and a set of angular momenta $J_r$, where $r = 1, \dots,rank[SO(D − 2)]$, and the horizon topology is $S^{D−2}$. In $D = 5$, for solutions which have
only one non-zero angular momentum $J_1 = J \neq 0$, they found the bound 
$J^2 \leq 32GM^3/(27\pi)$,
which is a generalisation of the known four dimensional Kerr bound $J \leq GM^2$. However for
$D > 5$, the momentum is unbounded, and the black hole can be ultra-spinning. Different black hole solutions can also have the same near-horizon geometry, for example in $D = 5$ the extremal self-dual Myers-Perry black hole and the extremal $J = 0$ Kaluza-Klein black hole.



\begin{comment}
Two black holes have the same masses, electrical charges, and angular momenta, but the first black hole is made out of ordinary matter whereas the second is made out of antimatter; nevertheless, they will be completely indistinguishable to an observer outside the event horizon. None of the special particle physics pseudo-charges (i.e., the global charges baryonic number, leptonic number, etc.) are conserved in the black hole
\end{comment}


\begin{comment}
In 1969, Roger Penrose proposes the cosmic censorship hypothesis. The weak and the strong cosmic censorship hypotheses are two mathematical conjectures about the structure of singularities arising in general relativity.

Singularities that arise in the solutions of Einstein's equations are typically hidden within event horizons, and therefore cannot be seen from the rest of spacetime. Singularities that are not so hidden are called naked. The weak cosmic censorship hypothesis was conceived by Roger Penrose in 1969 and posits that no naked singularities, other than the Big Bang singularity, exist in the universe.

The weak cosmic censorship hypothesis asserts there can be no singularity visible from future null infinity $\mathscr{I}^+$. In other words, singularities need to be hidden from an observer at infinity by the event horizon of a black hole. Mathematically, the conjecture states that, for generic initial data, the maximal Cauchy development possesses a complete future null infinity.

The strong cosmic censorship hypothesis asserts that, generically, general relativity is a deterministic theory, in the same sense that classical mechanics is a deterministic theory. In other words, the classical fate of all observers should be predictable from the initial data. Mathematically, the conjecture states that the maximal Cauchy development of generic compact or asymptotically flat initial data is locally inextendible as a regular Lorentzian manifold.


The two conjectures are mathematically independent, as there exist spacetimes for which weak cosmic censorship is valid but strong cosmic censorship is violated and, conversely, there exist spacetimes for which weak cosmic censorship is violated but strong cosmic censorship is valid.
\end{comment}

\subsection{The laws of black hole mechanics and entropy}
In 1972 Stephen Hawking proved that the area of a classical black hole's event horizon cannot decrease and along with James Bardeen, Brandon Carter \cite{bhmech}, they derived four laws of black hole mechanics in analogy with the laws of thermodynamics.

\begin{description} 
    \item[Zeroth Law:]
  \begin{description}
      The surface gravity $\kappa$
    is constant over the event horizon of a stationary black hole.
  \end{description}
    \item[First Law:]
  \begin{description}
    \[
    d M = \frac{\kappa}{8\pi}  d A + \Omega
    d J + \Phi d Q \ ,
    \]
    where $M$ is the total black hole mass, $A$ the surface area of
    the horizon, $\Omega$ is the angular velocity, $J$ is the angular momentum, $\Phi$ is the electrostatic potential and $Q$ is the electric charge. For the Reissner-Nordstr\"om black hole one has,
    \bea
    \kappa = \frac{r_+ - r_-}{2r_+^2}, ~\Phi = \frac{Q}{r_+},~ A = 4\pi r_+^2 \ ,
    \ee
  \end{description}
    \item[Second Law:]
  \begin{description}
     $d A \ge 0$
  \end{description}
    \item[Third Law:] 
  \begin{description}
    $\kappa = 0$ is not
    achievable by any physical process.
  \end{description}
\end{description}

Also in 1972, Jacob Bekenstein \cite{bekenstein} conjectured that black holes have an entropy proportional to their surface area due to information loss effects. In 1974, Stephen Hawking applied quantum field theory to black hole spacetimes and showed that black holes will radiate particles with a black-body spectrum which can cause black hole evaporation \cite{hradiation}. We can try to describe the interaction of some quantum matter with gravity by quantising the matter on a fixed, classical gravitational background. That is, we can try quantising the matter, but not the gravity. This will work only if the gravity is weak. It should work outside a large black hole, but not near the singularity. Using this approach, Hawking showed that a black hole will radiate thermally. That is, if we study quantum matter fields on a classical black hole background, we find that, when the matter fields are initially in the vacuum, there is a steady stream of outgoing radiation, which has a temperature determined by its mass and charge, which is surprising since classically, no radiation can escape from a black hole. This outgoing radiation, known as Hawking radiation, decreases the mass of the black holes, so eventually the black hole will disappear. The temperature goes up as the black hole gets smaller (unlike most things, which cool off as they lose energy), so the black hole will disappear abruptly, in a final flash of radiation. The black hole emits blackbody radiation with temperature
\bea
T_{BH} = \frac{\kappa\bar{h}}{2\pi} = \frac{\bar{h}c^3}{8\pi G M k_{B}} \ ,
\ee
where $\bar{h}$ is the reduced Planck constant, $c$ is the speed of light, $k_B$ is the Boltzmann constant, $G$ is the gravitational constant, and $M$ is the mass of the black hole. For the Reisnner-Nordstr\"om metric we have,
\bea
T_{RN} = \frac{\sqrt{M^2 - Q^2}}{2\pi(2M(M+ \sqrt{M^2 - Q^2}) - Q^2)} \ .
\ee
There is also an analogy between the classical laws governing black holes, and the laws of thermodynamics. Thermodynamics is just an approximate description of the behaviour of large groups of particles, which works because the particles obey statistical mechanics.  Since black holes have a non-zero temperature, the classical laws of black holes can be interpreted in terms of 
the laws of thermodynamics applied to black holes. We expect there to be
some more fundamental (quantum) description of black holes, which in particular would give some understanding of black hole microstates, whose statistical properties
give rise to the classical laws governing black holes in terms of statistical mechanics. The entropy of the black hole can be computed in terms of the area as;
\bea
S_{BH} = \pi r_{+}^2 = \frac{k_{B} A}{4 \ell^2_P} \ ,
\ee 
where $A$ is the area of the event horizon and $\ell_P = \sqrt{G\bar{h}/c^3}$ is the Planck length.  For the Reisnner-Nordstr\"om metric we have,
\bea
S_{RN} = \pi (M + \sqrt{M^2 -Q^2})^2 \ .
\ee
\begin{comment}
\subsection{Sagittarius A* 2002 2004}

Supermassive black hole are the largest type, on the order of hundreds of thousands to billions of solar masses, and are found in the centre of almost all currently known massive galaxies. Astronomers are still not sure how these supermassive black holes form. Just as stellar black holes result from the collapse of massive stars, some have suggested that supermassive black holes form out of the collapse of massive clouds of gas during the early stages of the formation of the galaxy.

All the stars in our galaxy or otherwise orbit a supermassive black hole at the centre of the galaxy they inhabit. Just as the moon orbits the earth and the earth orbits the sun, the sun (along with other stars in the Milky Way) also orbits the supermassive black hole at the centre of our Milky Way galaxy (Sagittarius A*).

\begin{figure}[h!]
  \includegraphics[width=250pt]{sgra.jpg}
  \caption{The center of the Milky Way galaxy, with the supermassive black hole Sagittarius A* (Sgr A*), located in the middle, is revealed in these images}
  \label{fig:sgra}
\end{figure}

Astronomers at the Max Planck Institute for Extraterrestrial Physics present evidence for the hypothesis that Sagittarius A* is a supermassive black hole at the center of the Milky Way galaxy in 2002. Further observations by a team from UCLA present even stronger evidence supporting Sagittarius A* as a black hole in 2004.

Astronomers have used NASA’s Chandra X-ray Observatory to take a major step in understanding why material around Sgr A* is extraordinarily faint in X-rays.
 
The large image in Figure \ref{fig:sgra} contains X-rays from Chandra in blue and infrared emission from the Hubble Space Telescope in red and yellow. The inset shows a close-up view of Sgr A* in X-rays only, covering a region half a light year wide. The diffuse X-ray emission is from hot gas captured by the black hole and being pulled inwards. This hot gas originates from winds produced by a disk-shaped distribution of young massive stars observed in infrared observations.

\subsection{First visual proof 2012}
First visual proof of existence of black-holes. Suvi Gezari's team in Johns Hopkins University, using the Hawaiian telescope Pan-STARRS 1, publish images of a supermassive black hole 2.7 million light-years away swallowing a red giant in 2012.
\begin{figure}[h!]
  \includegraphics[width=240pt]{visual.jpg}
  \caption{These images, taken with NASA's Galaxy Evolution Explorer and the Pan-STARRS1 telescope in Hawaii, show a brightening inside a galaxy caused by a flare from its nucleus. Image credit: NASA/JPL-Caltech/JHU/STScI/Harvard-Smithsonian CfA}
  \label{fig:visualproof}
\end{figure}
Figure \ref{fig:visualproof} above are images taken with NASA's Galaxy Evolution Explorer and the Pan-STARRS1 telescope in Hawaii, which show a brightening inside a galaxy caused by a flare from its nucleus. The arrow in each image points to the galaxy. The flare is a signature of the galaxy's central black hole shredding a star that wandered too close. 

The top left image, taken by the Galaxy Evolution Explorer in 2009, shows the galaxy's location before the flare. The galaxy is not visible in this ultraviolet-light exposure. In the top right image, taken by the Galaxy Evolution Explorer on June 23, 2010, the galaxy has become 350 times brighter in ultraviolet light. 

The bottom left image, taken by Pan-STARRS1, shows the galaxy (the bright dot in the center) in 2009 before the flare's appearance. The bottom right image, taken by Pan-STARRS1 from June to August 2010, shows the flare from the galaxy nucleus. Note how the light from the flare is much bluer, or hotter, than the host galaxy light. 
\end{comment}

\section{Symmetry in Physics}
At the centre of fundamental physics stands the concept of symmetry,
often implemented using the mathematics of group theory and Lie algebras.
A symmetry transformation is a mathematical transformation which leaves
all measurable quantities intact.  Spacetime symmetries correspond to transformations on a field theory acting explicitly on the spacetime coordinates
\bea
x^{\mu} \rightarrow x'^{\mu}(x^\nu),~~ \mu,\nu=0,1,2,\dots,d-1 \ .
\ee
A Killing vector is a coordinate
independent way of describing spacetime symmetries. There is a certain maximal
amount of symmetry that the geometry can have in a given number of
dimension, and the number of linearly independent Killing vectors $N \leq \frac{d(d-1)}{2}$ tells you what amount of symmetry you have. The space of all Killing vector fields form the Lie algebra ${\mathfrak{g}} = Lie(G)$ of the isometry group $G = Isom({\cal{M}})$ of a (semi) Riemanniann manifold $\cal{M}$. The group of isometries of a given connected smooth manifold is always a Lie group. However, a Lie group can include subgroups of discrete isometries that, barring the identity, cannot be represented by continuous isometries and thus they have no Killing vectors associated with them. For instance, referring to $\mathbb{R}^3$ equipped with the standard metric, the Lie group of isometries is the semidirect product of space translations $\mathbb{R}^3$ and rotations $O(3)$ around a fixed point. The second mentioned subgroup of isometries, $O(3)$, admits a discrete subgroup: $\{I,−I\}$. The spatial inversion $−I$ cannot be associated with any Killing field. 

Internal symmetries correspond to transformations of the different fields of the field theory,
\bea
\Phi^a (x) \rightarrow M^{a}{}_{b} \Phi^b (x) \ .
\ee
The indices $a, b$ label the corresponding fields. If $M^{a}{}_{b}$ is constant then then we have a global symmetry, if $M^{a}{}_{b}(x)$ is spacetime dependent then we have a local symmetry. The process of making a global symmetry into a local symmetry with $M^{a}{}_{b} \rightarrow M^{a}{}_{b}(x)$ is known as gauging. If the Lagrangian (or the action) of the theory is invariant under the symmetry
transformation we say that the theory has the symmetry. This doesn’t necessarily mean that the
solution has that symmetry - there are a variety of ways to break a
symmetry. Suffice to say, that the solution
has a symmetry if it is invariant under the symmetry transformation. Consider as an example the massless complex scalar field $\phi$ with Lagrangian,
\bea
\label{lagra1}
{\cal{L}} = \partial_{\mu}\phi \partial^{\mu}{\bar{\phi}} \ .
\ee
This theory has a $U(1)$ symmetry, acting as constant phase shift on the field $\phi$ as,
\bea
\label{sym}
\phi(x) \rightarrow e^{i \Lambda}\phi(x)
\ee
To construct a theory with local symmetry, we promote $\Lambda \rightarrow \Lambda(x)$ which allows the phase to depend on the space time coordinate. (\ref{sym}) is no longer a symmetry of the Lagrangian (\ref{lagra1}), in order to repair the symmetry we need to introduce the covariant derivative of a gauge field over the spacetime manifold,
\bea
D_{\mu}\phi(x) \equiv \partial_{\mu}\phi(x) -i A_{\mu} \phi(x)
\ee
and replace ordinary derivative with this covariant derivative in the Lagrangian (\ref{lagra1}) to get,
\bea
{\cal{L}} = D_{\mu}\phi D^{\mu}{\bar{\phi}} \ .
\ee


\subsection{Noether's theorem}
Noether's theorem, which was proven by Emmy Noether in 1915, states that every differentiable symmetry of the action of a physical system has a corresponding conservation law \cite{noether}. Noether's theorem relates the global symmetries of the action to the conservation laws. It is interesting that the actions used in the original work can have any number of derivatives and still under certain conditions specified one finds a conservation of the Noether current, once the Euler-Lagrange field equations are satisfied, even when the relevant actions have an infinite number of derivatives. Noether transformations laws acting on the fields can be linear or nonlinear, or some combination of these. 

As a consequence of Noether's theorem, symmetries label and classify particles according to the different conserved quantum numbers identified by the spacetime and internal symmetries (mass, spin, charge, colour, etc.). In this regard symmetries actually define an elementary particle according to the behaviour of the corresponding field with respect to the corresponding symmetry. This property was used to classify particles not only as fermions and bosons but also to group them in multiplets.

\begin{comment}
\subsection{Killing vectors}
\subsection{Lie derivative}
\subsection{Lie algebra}
\end{comment}

\subsection{Poincar\'e symmetry}
The Poincare group corresponds to the basic symmetries of special relativity, it acts on spacetime coordinates $x^\mu$ as follows:
\bea
x^{\mu} \rightarrow x'^{\mu} = \Lambda^{\mu}{}_{\nu} x^{\nu} + a^\mu \ ,
\ee
where $\Lambda^{\mu}{}_{\nu}$ correspond to the Lorentz transformations, and $a^{\mu}$ the translations. The Poincaré algebra is the Lie algebra of the Poincaré group. More specifically, the proper ($\det \Lambda =1$), orthochronous ($\Lambda^{0}{}_{0} \geq 1$) part of the Lorentz subgroup, $SO^+(1, 3)$, connected to the identity. Generators for the Poincaré group are $M_{\mu \nu}$ and $P_{\mu}$ and the Poincare algebra is given by the commutation relations:
\bea
[P_\mu, P_\nu] &=& 0 \ ,
\cr
[M_{\mu \nu}, P_{\rho}] &=& i(\eta_{\mu \rho}P_{\nu} - \eta_{\nu \rho}P_{\mu}) \ ,
\cr
[M_{\mu \nu}, M_{\rho \sigma}] &=& i(\eta_{\mu \rho}M_{\nu \sigma} - \eta_{\mu \sigma}M_{\nu \rho} - \eta_{\nu \rho}M_{\mu \sigma} + \eta_{\nu \sigma}M_{\mu \rho}) \ .
\ee

To include new symmetries we extend the Poincar\'e group via new anticommuting
symmetry generators, and postulate their anticommutation relations. To
ensure that these unobserved symmetries do not conflict with experimental results
obtained thus far we must assume that supersymmetry is spontaneously broken,
allowing the superpartners to be more massive than the energy scales probed thus
far.


\section{Quantum gravity}
\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=350pt]{qg.png}
	\end{center}
	\caption{Diagram showing where quantum gravity sits in the hierarchy of physical theories (credit: \url{https://goo.gl/9RmT3Z})}
	\label{fig:qg}
\end{figure}
Quantising matter fields on a black hole background teaches us a lot about black holes. However, we need a quantum theory of gravity to understand the fundamental principles underlying black hole thermodynamics. We also need a quantum theory to tell us what happens near the singularity.  On short distance scales, we certainly need to use a quantum theory to describe the collapsing matter as general relativity provides no basis for working out what happens next. When you reach the singularity, the equations no longer make sense or have any predictive power. It is hoped that this failure of the classical theory can be cured by quantising gravity as well. A complete quantum theory of gravity would also be able
to explain the nature of the end-point of black 
hole evaporation. The same problem crops up when trying to explain the big bang, which is thought to have started with a singularity. 
\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=430pt]{toe.png}
	\end{center}
	\caption{Theory Of Everything}
	\label{fig:toe}
\end{figure}

Another motivation for quantum gravity would be for the unification of the laws of nature. The standard model describes strong, weak and electromagnetic force with gauge group $SU(3) \times SU(2) \times U(1)$ and the experimental verification of quantum electrodynamics has been the most stringently tested theories in physics. General relativity which describes gravity is another theory which has been rigorously tested in the very strong field limit, observing to date no deviations from the theory. Naive attempts at reconciling these theories have failed, yet a true unified theory of everything must include all the forces of nature. In Figure \ref{fig:toe}, each unification step leads one level up and electroweak unification occurs at around 100 GeV, grand unification is predicted to occur at 1016 GeV, and unification of the GUT force with gravity is expected at the Planck energy, roughly 1019 GeV.

Formulating a theory of quantum gravity has turned out to be one of the hardest problems of modern physics. Attempts to incorporate gravity into the quantum framework as if it were just another force like electromagnetism or the nuclear forces have failed; such models are riddled with infinities and do not make any sense physically. Until now, the question of how a proper quantum theory of gravity should look has not found a complete answer.  One theory which offers some hope, particularly for understanding black holes, is string theory. 

%Four fundamental forces of nature: Strong, Weak, Electromagnetism and Gravity. Standard model gauge group $SU(3) \times SU(2) \times U(1)$.

\subsection{Kaluza-Klein unification and compactification}
\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=150pt]{KK.png}
	\end{center}
  \caption{Kaluza-Klein compactification (credit: \url{https://goo.gl/cXymk1})}
  \label{fig:KK}
\end{figure}
In physics, Kaluza-Klein theory is a classical unified field theory of gravitation and electromagnetism. The crucial idea of compactificaton built around the idea of a fifth dimension beyond the usual four of space and time is considered an important precursor to string theory and supergravity. Compactification is one way of modifying the number of dimensions in a physical theory. In compactification, some of the extra dimensions are assumed to ``close up" on themselves to form circles. In the limit where these curled up dimensions become very small, one obtains a theory in which spacetime effectively has a lower number of dimensions. 

The original idea came from Theodor Kaluza in 1919, which detailed an extension of general relativity to five dimensions \cite{kaluza}. The metric for this theory ${\hat g}_{A B}$ has 15 components, ten components are identified with the four-dimensional spacetime metric $g_{\mu \nu}$, four components with the electromagnetic vector potential $A_{\mu}$, and one component with an unidentified scalar field $\Phi$ sometimes called the ``dilaton". More precisely we have,
\bea
{\hat g}_{\mu \nu} = g_{\mu \nu} + \Phi^2 A_{\mu} A_{\nu},~~ {\hat g}_{5 \nu} = {\hat g}_{\nu 5} = \Phi^2 A_{\nu},~~ {\hat g}_{5 5} = \Phi^2 \ .
\ee
Kaluza also introduced the ``cylinder condition", which states that no component of the five-dimensional metric depends on the fifth dimension. Without this assumption, the field equations of five-dimensional relativity become intractable as they grow in complexity. The five-dimensional Einstein equations yield the four-dimensional Einstein field equations, the Maxwell equations for the electromagnetic field $A_{\mu}$, and an equation for the scalar field $\Phi$ given by,
\bea
R_{\mu \nu} - \frac{1}{2}g_{\mu \nu}R &=& \frac{1}{2}\Phi^2 \bigg(F_{\mu \alpha}F_{\nu}{}^{\alpha} - \frac{1}{4}F_{\alpha \beta}F^{\alpha \beta}\bigg) + \Phi^{-1}\bigg(\nabla_{\mu}\nabla_{\nu} \Phi - g_{\mu \nu}\nabla^{\lambda}\nabla_{\lambda}\Phi \bigg) \ ,
\cr
\nabla^{\beta}( \Phi^3 F_{\alpha \beta} )&=& 0 \ ,
\cr
\nabla^{\mu}\nabla_{\mu} \Phi  &=& \frac{1}{4}\Phi^3 F_{\alpha \beta}F^{\alpha \beta} \ .
\ee
The Einstein equation and field equation for $A_{\mu}$ has the form of the vacuum Maxwell equations if the scalar field is constant. It turns out that the scalar field cannot be set to a constant without constraining the electromagnetic field $A_{\mu}$. The earlier treatments by Kaluza and Klein did not have an adequate description of the scalar field $\Phi$, and did not realize the implied constraint.

\subsection{Supersymmetry}
\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=250pt]{susy.png}
	\end{center}
	\caption{The Standard Model and Supersymmetry (credit: \url{https://goo.gl/QcqXih})}
	\label{fig:susy}
\end{figure}
One attractive solution to the dark matter problem is supersymmetry. As
a consequence of supersymmetry, all fermion particles get their own boson
superpartner, and all boson particles get their own fermion superpartner.
It turns out that it is possible to have symmetry
transformations where the symmetry parameter is not a phase shift or some
other such Lorentz scalar, but actually a spinor. The matter fields of the fermions are spinors, so when we take the symmetry parameter to be a spinor, the symmetry transformation necessarily relates the bosons to fermions, and vice versa. Schematically this can be represented as,
\bea
\delta_1 B = \bar{\epsilon_1}F,~~
\delta_2 F = \partial B \epsilon_2 \ ,
\ee
where $F$ and $B$ denote the fermionic and bosonic fields respectively. The anticommuting parameter $\epsilon$ known as a spinor must have dimension $[\epsilon] = -\frac{1}{2}$ in mass units since $[B] =1$ and $[F] = \frac{3}{2}$, which implies the presence of the derivative operator in the second transformation to ensure dimensional consistency. If we consider the effect of successive supersymmetry variations,
\bea
\{\delta_1, \delta_2 \} = a^{\mu}\partial_{\mu}B,~~ a^{\mu} = \epsilon_2 \gamma^{\mu} {\bar{\epsilon}}_1
\ee
Supersymmetry is not just a symmetry between bosons and fermions, it is also an extension of the Poincar\'e symmetry, which is the symmetry of Minkowski spacetime. When talking about supersymmetry, one frequently considers rigid supersymmetry which is a global symmetry, whose symmetry parameters do not
depend on the point in spacetime. If we gauge it and make the global symmetry into a local one with $\epsilon \rightarrow \epsilon(x)$, it is possible to supersymmetrize general relativity by combining the standard bosonic metric 
with a gravitino, as well as more general bosonic and fermionic matter terms.

 For this reason, rather than talking about local supersymmetry or gauged supersymmetry, the established term is supergravity.  In supergravity theories, the vanishing of the supersymmetry variations when we set the fermions to zero are known as the Killing spinor equations (KSEs). Similarly
to symmetry, there is a maximum amount of possible supersymmetry, and the number of linearly independent Killing spinors determines how much of that supersymmetry is realised for a given bosonic solution. 




\subsection{Super-poincar\'e symmetry}
In order to have a supersymmetric extension of the Poincar\'e algebra, we first introduce graded algebras. Let ${\cal O}_a$ be operators of a Lie algebra, then
\bea
{\cal O}_a {\cal O}_b = (-1)^{\eta_a \eta_b} {\cal O}_b {\cal O}_a = iC^{e}{}_{a b}{\cal O}_e \ ,
\ee
where the gradings take the values $\eta_a = 0$ for a bosonic generator ${\cal O}_a$ and $\eta_a = 1$ for a fermionic generator ${\cal O}_a$. For supersymmetry, generators are the Poincar\'e generators $M_{\mu \nu}$, $P_{\mu}$ and the spinor generators $Q^{A}_{\alpha}$, ${\bar{Q}}^{A}_{{\dot \alpha}}$ where $A=1,\dots,\cal{N}$.
The simplest supersymmetric extension with ${\cal N} = 1$ is defined by the following commutation relations,
\bea
[Q_{\alpha}, P^{\mu}] &=& 0 \ ,
\cr
\{Q_{\alpha}, {\bar{Q}}_{{\dot \beta}} \} &=& 2 (\sigma^\mu)_{\alpha {\dot \beta}} P_{\mu} \ ,
\ee
where $P_{\mu}$ are the generators of translation as before and $\sigma^\mu$ are Pauli matrices. As before $\mu$ is a spacetime index, but $\alpha$ is a spinor index and has $\alpha = 1,2$ where a dot over the index transforms according to an inequivalent conjugate spinor representation. Combined with the Poincar\'e algebra, this is a closed algebra since all the super-Jacobi identities are satisfied. 
For the case of ${\cal N} > 1$, it is known as extended supersymmetry where each of the generators will be labelled by the index $A$ and will contain additional (anti)-commutation relations with central charges $Z^{A B}$ given by,
\bea
\{Q_{\alpha}^{A}, {\bar{Q}}_{{\dot \beta}}^B \} &=& 2 (\sigma^\mu)_{\alpha {\dot \beta}} P_{\mu} \delta^{A B} \ ,
\cr
\{Q_{\alpha}^{A},Q_{\beta}^B \} &=& \epsilon_{A B}Z^{A B} \ .
\ee
The central charges are anti-symmetric $Z^{A B} = -Z^{B A}$ and commute with all the generators. For model building, it has been assumed that almost all the supersymmetries would be broken in nature leaving just ${\cal{N}}=1$ supersymmetry.



\subsection{Superstring theory}

In physics, string theory is a theoretical framework in which the point-like particles of particle physics are replaced by one-dimensional objects called strings. It describes how these strings propagate through space and interact with each other. On distance scales larger than the string scale, a string looks just like an ordinary particle, with its mass, charge, and other properties determined by the vibrational state of the string. In string theory, one of the many vibrational states of the string corresponds to the graviton, a quantum mechanical particle that carries gravitational force. Thus string theory is a theory of quantum gravity. String theory was first studied in the late 1960s as a theory of the strong nuclear force, before being abandoned in favor of quantum chromodynamics. Subsequently, it was realized that the very properties that made string theory unsuitable as a theory of nuclear physics made it a promising candidate for a quantum theory of gravity. 

The earliest version of string theory known as bosonic string theory was discovered by John H. Schwarz and Joel Scherk \cite{schwarz}, and independently Tamiaki Yoneya, \cite{yoneya} in 1974. They studied the boson-like patterns of string vibration and found that their properties exactly matched those of the graviton. 
We recall that the dynamics of a point-like particle of mass $m$ moving in Minkowski spacetime is described by the action,
\bea
S = -m \int ds \ .
\ee
Consider now a string of lenth $\ell_s$ moving in Minkowski spacetime. The dynamics is governed by the Nambu-Goto action,
\bea
S = -T \int d{\cal A} \ ,
\ee
where $d{\cal A}$ is the infinitestimal area element of the string world-sheet. The Polyakov action which is classically equivalent, describes a two-dimensional sigma model given by,
\bea
S = -T\int d^2\sigma \sqrt{-\gamma} \gamma^{a b}g_{\mu \nu}\nabla_{a}X^{\mu} \nabla_{b}X^{\nu}
\ee
where $\sigma^a$ are coordinates on the string world-sheet with metric $\gamma_{a b}$ and spacetime metric $g_{\mu \nu}$. The requirement that unphysical states with negative norm disappear implies that the dimension of spacetime be 26, a feature that was originally discovered by Claud Lovelace in 1971 \cite{lovelace} but the open string spectrum still contained a tachyon as a ground state. Furthermore, any unified theory of physics should also contain fermions and it turns out including fermions provides a way to eliminate the tachyon from the spectrum. Investigating how a string theory may include fermions in its spectrum led to the invention of supersymmetry \cite{gervais}. It was later developed into superstring theory and its action looks like,
\bea
S = -T\int d^2\sigma \sqrt{-\gamma}\bigg(\gamma^{a b}g_{\mu \nu}\nabla_{a}X^{\mu} \nabla_{b}X^{\nu} - i g_{\mu \nu}{\bar \psi}^{\mu}\Gamma^{a}\nabla_{a} \psi^{\nu} \bigg) \ ,
\ee
where $\psi^{\mu}$ is a fermion, and $\Gamma^{a}$ the gamma matrices in the 2-dimensional world-sheet. Quantum mechanical consistency now requires that the dimension of spacetime be 10 for superstring theory, which had been originally discovered by John H. Schwarz in 1972 \cite{schwarz2}. 

Consider a closed bosonic string in a more general background consisting of massless states $(\Phi, h_{\mu \nu}, B_{\mu \nu})$ generated by closed strings in the bulk. The resulting action is called the non-linear sigma model,
\bea
S = -T\int d^2\sigma \bigg[\bigg(\sqrt{-\gamma} \gamma^{a b}g_{\mu \nu} - \epsilon^{a b}B_{\mu \nu}\bigg)\nabla_{a}X^{\mu} \nabla_{b}X^{\nu} - \alpha' \sqrt{-\gamma} \Phi {\cal {R}}^{(2)}\bigg] \ ,
\ee
where the background metric is given by $g_{\mu \nu} = \eta_{\mu \nu} + h_{\mu \nu}$ and ${\cal {R}}^{(2)}$ is the Ricci-scalar of the worldsheet metric $\gamma$. The $\beta$-functionals associated to the "coupling constants" $\Phi$, $h_{\mu \nu}$ and $B_{\mu \nu}$ vanish and in the lowest order in $\alpha'$ are given by \cite{callan},
\bea
\beta^{(\Phi)} &=& R + \frac{1}{12}H_{\mu \nu \rho}H^{\mu \nu \rho} - 4\nabla^{\rho}\nabla_{\rho}\Phi + 4 \nabla^{\rho}\Phi \nabla_{\rho}\Phi + O(\alpha')= 0 \ ,
\nonumber \\
\beta^{(h)}_{\mu \nu} &=& R_{\mu \nu} - \frac{1}{4}H_{\mu \rho \sigma}H_{\nu}{}^{\rho \sigma} + 2 \nabla_{\mu}\nabla_{\nu} \Phi + O(\alpha') = 0 \ ,
\nonumber \\
\beta^{(B)}_{\mu \nu} &=& \frac{1}{2}\nabla^{\rho}H_{\rho \mu \nu} - H_{\mu \nu \rho}\nabla^{\rho}\Phi + O(\alpha') = 0 \ ,
\ee
where $R_{\mu \nu}$ is the Ricci tensor of the space-time, and $H_{\mu \nu \rho} = 3\nabla_{[\mu}B_{\nu \rho]}$. The form of these equations suggests they can be interpreted as equations of motion for the background fields. Indeed they can also be obtained from the following low energy effective action,
\bea
\label{laction}
S = \int d^{26} x \sqrt{-g} e^{-2\Phi}\bigg(R + 4\nabla^{\mu}\nabla_{\mu}\Phi - \frac{1}{12}H_{\mu \nu \rho}H^{\mu \nu \rho} + O(\alpha')\bigg) \ .
\ee
So far this is only for bosonic string theory and in $D=26$, but this can be extended to the supersymmetric case in $D=10$. It turns out that the low energy effective descriptions of superstring theories in $D=10$, except type I, have one part in common known as the `common sector', which is the NS-NS sector given by the ten dimensional analogue of (\ref{laction}). Five consistent versions of superstring theory were developed before it was conjectured in the mid-1990s that they were all different limiting cases of a single theory in eleven dimensions known as M-theory. In late 1997, theorists discovered an important relationship called the AdS/CFT correspondence, which relates string theory to certain quantum field theories and has also led to many insights in pure mathematics. The low energy limits of these superstring theories coincide with supergravity. In 1978, $D=11$ was shown to be the largest number of dimensions consistent with a single graviton in supergravity theories \cite{nahm}. 


\subsubsection{The first superstring revolution}
The first superstring revolution is a period of important discoveries that began in 1984. The revolution was started by a discovery of anomaly cancellation in type I string theory via the Green-Schwarz mechanism  in 1984 \cite{green}. The ground-breaking discovery of the heterotic string was made by David Gross, Jeffrey Harvey, Emil Martinec, and Ryan Rohm in 1985 \cite{gross}. It was also realized by Philip Candelas, Gary Horowitz, Andrew Strominger, and Edward Witten in 1985 that to obtain $N=1$ supersymmetry, the six small extra dimensions  need to be compactified on a Calabi-Yau manifold \cite{candelas}. By 1985, five separate superstring theories had been described: type I, type II (IIA and IIB) \cite{green2}, and heterotic ($SO(32)$ and $E_8 \times E_8$) \cite{gross}.  In 1987, Eric Bergshoeff, Ergin Sezgin and Paul Townsend showed that there are no superstrings in eleven dimensions, but supermembranes \cite{bergshoeff}.

\subsubsection{The second superstring revolution}

In the early 1990s, Edward Witten and others found strong evidence that the different superstring theories were different limits of an 11-dimensional theory that became known as M-theory \cite{witten2, duff}. These discoveries sparked the second superstring revolution that took place approximately between 1994 and 1995. The different versions of superstring theory were unified, as long hoped, by new equivalences. These are known as S-duality, T-duality, U-duality, mirror symmetry, and conifold transitions. The different theories of strings were also related to M-theory.

\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=250pt]{d-brane.png}
	\end{center}
	\caption{Open strings attached to a pair of D-branes (credit: \url{https://goo.gl/nvdmgM})}
	\label{fig:dbrane}
\end{figure}

In 1995, Joseph Polchinski discovered that the theory requires the inclusion of higher-dimensional objects, called D-branes\footnote{The letter "D" in D-brane refers to a certain mathematical condition on the system known as the Dirichlet boundary condition.} \cite{polchinski}: these are the sources of electric and magnetic Ramond–Ramond fields that are required by string duality. A brane is a physical object that generalizes the notion of a point particle to higher dimensions. For instance, a point particle can be viewed as a brane of dimension zero, while a string can be viewed as a brane of dimension one. It is also possible to consider higher-dimensional branes. In dimension $p$, these are called $p$-branes. The word brane comes from the word ``membrane" which refers to a two-dimensional brane.

Branes are dynamical objects which can propagate through spacetime according to the rules of quantum mechanics. They have mass and can have other attributes such as charge. A $p$-brane sweeps out a $(p+1)$-dimensional volume in spacetime called its world volume. In string theory, D-branes are an important class of branes that arise when one considers open strings. As an open string propagates through spacetime, its endpoints are required to lie on a D-brane. The study of D-branes in string theory has led to important results such as the AdS/CFT correspondence, which has shed light on many problems in quantum field theory. D-branes added additional rich mathematical structure to the theory, and opened possibilities for constructing realistic cosmological models. In 1997–98, Juan Maldacena conjectured a relationship between string theory and $N = 4$ supersymmetric Yang–Mills theory, a gauge theory \cite{maldacena, maldacena2}. This conjecture, called the AdS/CFT correspondence, has generated a great deal of interest in high energy physics. It is a realization of the holographic principle, which has far-reaching implications: the AdS/CFT correspondence has helped elucidate the mysteries of black holes suggested by Stephen Hawking's work and is believed to provide a resolution of the black hole information paradox \cite{maldacena3}.


\begin{comment}
\begin{figure}[h!]
  \includegraphics[width=250pt]{worldsheet.png}
  \caption{Wiki: World line, worldsheet, and world volume, as they are derived from particles, strings, and branes.}
  \label{fig:worldsheet}
\end{figure}
\end{comment}


\section{Supergravity}
Supergravity is often called a ``square root" of General Relativity. Indeed,
a supersymmetric extension of the Poincar\'e algebra is reminiscent of Dirac's procedure of
obtaining a spin $1/2$ wave equation from the scalar wave equation. Supergravity has played an important role in theoretical high-energy physics since it began, merging the theory of general relativity and supersymmetry. In fact, supergravity arises naturally when we promote  supersymmetry to a local (gauge) symmetry \cite{wess}. A bosonic sector of
extended supergravities, apart from the graviton, contains scalar and vector fields. In ${\cal N} = 2, D=4$ supergravity, the bosonic sector is the usual Einstein-Maxwell theory. Supergravity is also understood to be the low-energy limit of string theory, that is if we truncate to the massless modes. In Supergravity theories, Supersymmetry transformations are generated by a set of spinors $\epsilon_{I}(x)$ for $I = 1,\dots\,{\cal{N}}$, where ${\cal{N}}$ is the number of supersymmetries of the given Supergravity. In $D=4$, the spinors $\epsilon_{I}(x)$ can be taken to be Weyl or Majorona, and we have $2{\cal{N}}$ complex or $4{\cal{N}}$ real associated charges. Such transformations schematically have the form \cite{wess2, volkov, akulov},
\bea
\delta B = \bar{\epsilon}(B + \bar{F}F)F,~~ \delta F = \partial \epsilon + (B + \bar{F}F) \epsilon F \ ,
\ee
where $F$ and $B$ denote the fermionic and bosonic fields respectively. Since all Supergravity theories will contain at least a graviton $g$, which is a bosonic field, it will also have a corresponding gravitino $\psi$, which is a fermionic field. Such theories will have the transformations,
\bea
\delta e^{a}_{M} = \alpha \bar{\epsilon} \Gamma^a\psi_{M},~~ \delta \psi_{M} = \nabla_{M} \epsilon + \Psi_{M}\epsilon,~~ \alpha \in \mathbb{C} \ ,
\ee
and possibly additional transformations for the other bosonic and fermionic fields of the supergravity theory in question, where $\alpha$ depends on the particular supergravity and $\Psi_M$ depends on the fluxes of that theory. When looking for classical supergravity solutions, we will not get any constraints from the variation of the bosons since these pertain to vanishing fermion fields and become trivial, but the variation of fermions gives us differential and possibly algebraic equations for the spinor $\epsilon$ which are called Killing spinor equations (KSEs) and take the form,
\bea
\delta \psi_M \equiv {\cal{D}}_{M}\epsilon = 0,~~ \delta \lambda_I \equiv {\cal{A}}_I \epsilon = 0 \ ,
\ee
where ${\cal{D}}_{M}$ is known as the supercovariant derivative and $\delta \lambda_I$ collectively denote the variations of the additional fermions in theory pertaining to the algebraic conditions. The integrability conditions of the KSEs of a particular Supergravity theory can also be written in terms of the field equations and Bianchi identities of that theory. Also, if $\epsilon$ is a killing spinor, one can show for all supergravity theories using a spin-invariant inner product that,
\bea
K =  \langle \epsilon, \Gamma^{\mu} \epsilon \rangle \partial_{\mu} \ ,
\ee
is a killing vector. If we take the inner product given by $\langle \epsilon, \Gamma_{\mu} \epsilon \rangle = \bar{\epsilon}\Gamma_{0}\Gamma_{\mu}\epsilon$, then the vector $K$ is always non-vanishing. As an example, let us consider these for Heterotic supergravity; the bosonic fields are the metric $g$, a dilaton field $\Phi$, a 3-form $H$ and a non-abelian 2-form field $F$ and the fermionic fields are the gravitino $\psi_{\mu}$, the dilatino $\lambda$ and gaugino $\chi$ which we set to zero. 
Let us first consider the integrability conditions for the KSEs. The field equations and Bianchi identities are,
\bea
E_{\mu \nu} &=& R_{\mu \nu} + 2 \nabla_\mu \nabla_\nu \Phi
-{1 \over 4} H_{\mu \lambda_1 \lambda_2} H_\nu{}^{\lambda_1 \lambda_2} = 0 \ ,
\nonumber \\
F\Phi &=& \nabla^\mu \nabla_\mu \Phi
- 2 \nabla_\lambda \Phi \nabla^\lambda \Phi
+{1 \over 12} H_{\lambda_1 \lambda_2 \lambda_3}H^{\lambda_1 \lambda_2 \lambda_3} = 0 \ ,
\nonumber \\
FH_{\mu \nu} &=& \nabla^{\rho}(e^{-2\Phi}H_{\mu \nu \rho}) = 0 \ ,
\nonumber \\
FF_{\mu} &=& \nabla^{\nu}(e^{-2\Phi}F_{\mu \nu}) - \frac{1}{2}e^{-2\Phi}H_{\mu \nu \rho}F^{\nu \rho} = 0 \ ,
\nonumber \\
BH_{\mu \nu \rho \sigma} &=& \nabla_{[\mu}H_{\nu \rho \sigma]} = 0 \ ,
\nonumber \\
BF_{\mu \nu \rho} &=& \nabla_{[\mu}F_{\nu \rho]} = 0 \ ,
\ee
and the KSEs are,
\bea
{\cal D}_{\mu}\epsilon &=& \nabla_{\mu}\epsilon - \frac{1}{8}H_{\mu \nu \rho}\Gamma^{\nu \rho}\epsilon = 0 \ ,
\nonumber \\
{\cal{A}}\epsilon &=& \nabla^{\mu}{\Phi}\Gamma^{\mu}\epsilon - \frac{1}{12}H_{\mu \nu \rho}\Gamma^{\mu \nu \rho}\epsilon = 0 \ ,
\nonumber \\
{\cal {F}}\epsilon &=& F_{\mu \nu}\Gamma^{\mu \nu}\epsilon = 0 \ ,
\ee
The integrability conditions of the KSEs can be expressed in terms of the field equations and Bianchi identities as follows,
\bea
\Gamma^{\nu}[{\cal{D}}_{\mu},{\cal{D}}_{\nu}]\epsilon - [{\cal{D}}_{\mu},{\cal{A}}]\epsilon &=& \bigg(-\frac{1}{2}E_{\mu \nu}\Gamma^{\nu}  - \frac{1}{4}e^{2\Phi}FH_{\mu \nu}\Gamma^{\nu} - \frac{1}{6}BH_{\mu \nu \rho \lambda}\Gamma^{\nu \rho \lambda} \bigg)\epsilon \ ,
\nonumber \\
\Gamma^{\mu}[{\cal{D}}_{\mu},{\cal{A}}]\epsilon - 2{\cal{A}}^2 \epsilon &=& \bigg(F\Phi - \frac{1}{4}e^{2\Phi}FH_{\mu \nu}\Gamma^{\mu \nu} - \frac{1}{12}BH_{\mu \nu \rho \lambda}\Gamma^{\mu \nu \rho \lambda}\bigg)\epsilon \ ,
\nonumber \\
\Gamma^{\mu}[{\cal{D}}_{\mu}, {\cal{F}}]\epsilon + [{\cal{F}},{\cal{A}}]\epsilon &=& \bigg(-2e^{2\Phi}FF_{\mu}\Gamma^{\mu} + BF_{\mu \nu \rho}\Gamma^{\mu \nu \rho}\bigg)\epsilon \ .
\ee
To show that $K$ is a killing vector in heterotic supergravity, we consider the supercovariant derivative for a 1-form $K_{\mu}$ is given by,
\bea
{\cal D}_{\mu}K_{\nu} = \nabla_{\mu}K_{\nu} + \frac{1}{2}H_{\mu \nu}{}^{\rho}K_{\rho} \ .
\ee
If we compute the supercovariant derivative directly from the inner product we have,
\bea
{\cal D}_{\mu}K_{\nu} = {\cal D}_{\mu} \langle \epsilon, \Gamma_{\nu} \epsilon \rangle = \langle {\cal D}_{\mu}\epsilon, \Gamma_{\nu} \epsilon \rangle + \langle \epsilon, \Gamma_{\nu} {\cal D}_{\mu}\epsilon \rangle = 0 \ ,
\ee
since $\epsilon$ is a killing spinor, this implies,
\bea
\nabla_{\mu}K_{\nu} = -\frac{1}{2}H_{\mu \nu}{}^{\rho}K_{\rho} \ ,
\ee
and hence $K$ is a killing vector since $H$ is skew-symmetric and we have,
\bea
\nabla_{(\mu}K_{\nu)} = 0 \ .
\ee

One of the most interesting bosonic structures is suggested by $N = 4$ supergravity, which attracted attention in connection with ``stringy" black holes. Investigations into supergravity first began in the mid 1970's through the work
of Freedman, Van Nieuwenhuizen and Ferrara, at around the time that the implications
of supersymmetry for quantum field theory were first beginning to be
understood \cite{freedman}. 

\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=300pt]{mtheory.png}
	\end{center}
	\caption{A schematic illustration of the relationship between M-theory, the five superstring theories, and eleven-dimensional supergravity. (credit: \url{https://goo.gl/5Q4Aw4})}
	\label{fig:sugras}
\end{figure}

Supergravity means that we have a symmetry whose symmetry parameter is a spinor that depends on the position in the spacetime. We are looking for supersymmetric geometries, and we get them by insisting
that the solution is invariant under the supersymmetry transformation and if it is we call the supersymmetry parameter a Killing spinor. On a bosonic background, the Killing spinor is solution to the KSEs, which are given by demanding that the fermions vanish. In the limit where quantum gravity effects are small, the superstring theories which are related by certain limits and dualities, give rise to different types of supergravity.
The focus of this work has been type IIA, massive IIA and $D=5$ (gauged and ungauged) supergravity coupled to an arbitrary number of vector multiplets. Type IIA supergravity is
a ten-dimensional theory which can be obtained either by taking a certain limit in type IIA string theory, or by doing a dimensional reduction of $D=11$ supergravity on $S^1$. $D=5$ ungauged supergravity can be obtained from reducing $D=11$ supergravity on a $T^6$, or more generally a Calabi-Yau compactification \cite{cadavid} and $D=5$ gauged supergravity can be obtained from reducing IIB supergravity on $S^5$ \cite{gutperle}.


\subsection{$D=4, N=8$ supergravity}
In 4 spacetime dimensions, $N=8$ Supergravity is the most symmetric quantum field theory which involves gravity and a finite number of fields. It can be found from a dimensional reduction of 11D supergravity by making the size of 7 of the dimensions go to zero. It has 8 supersymmetries (maximally supersymmetric) which is the most any gravitational theory can have. The theory was found to predict rather than assume the correct charges for fundamental particles, and potentially offered to replicate much
of the content of the standard model \cite{vannie} and Stephen Hawking once speculated that this theory could be the Theory of Everything \cite{hawkingd4n8}. This optimism however proved to be short lived, and in
particular it was not long before a number of gauge and gravitational anomalies
were discovered; seemingly fatal flaws which would render the theory inconsistent \cite{green}. In later years this was initially abandoned in favour of String Theory. There has been renewed interest in the 21st century with the possibility that the theory may be finite. 

\subsection{$D=11, N=1$ supergravity}
One of these supergravities, the 11-dimensional theory, generated considerable excitement as the first potential candidate for the theory of everything. Werner Nahm showed $11$ dimensions as the largest number of dimensions consistent with a single graviton, and more dimensions will show particles with spins greater than 2 \cite{nahm}. In 1981 Edward Witten also showed 11 as the smallest number of dimensions big enough to contain the gauge groups of the Standard Model, namely $SU(3)$ for the strong interactions and $SU(2) \times U(1)$ for the electroweak interactions \cite{witten}. Many techniques exist to embed the standard model gauge group in supergravity in any number of dimensions like the obligatory gauge symmetry in type I and heterotic string theories, and obtained in type II string theory by compactification on certain Calabi–Yau manifolds. The D-branes engineer gauge symmetries too. In 1978 Cremmer, Julia and Scherk (CJS) found the classical action for an 11-dimensional supergravity theory \cite{cremmer}. This remains today the only known classical 11-dimensional theory with local supersymmetry and no fields of spin higher than two. Other 11-dimensional theories known and quantum-mechanically inequivalent reduce to the CJS theory when one imposes the classical equations of motion.  In 1980 Peter Freund and M. A. Rubin showed that compactification from 11 dimensions preserving all the SUSY generators could occur in two ways, leaving only 4 or 7 macroscopic dimensions, the others compact \cite{rubin}. The noncompact dimensions have to form an anti-de Sitter space. There are many possible compactifications, but the Freund-Rubin compactification's invariance under all of the supersymmetry transformations preserves the action. Finally, the first two results each appeared to establish 11 dimensions, the third result appeared to specify the theory, and the last result explained why the observed universe appears to be four-dimensional. For $D=11$ supergravity, the field content only contains the graviton, the gravitino and a 3-form potential $A^{(3)}$.

Initial excitement about the 10-dimensional theories, and the string theories that provide their quantum completion, died by the end of the 1980s. There were too many Calabi–Yaus to compactify on, many more than Yau had initially estimated in 2005. None quite gave the standard model, but it seemed as though one could get close with enough effort in many distinct ways. Plus no one understood the theory beyond the regime of applicability of string perturbation theory. There was a comparatively quiet period at the beginning of the 1990s although several important tools were developed. For example, it became apparent that the various superstring theories were related by "string dualities", some of which relate weak string-coupling - perturbative - physics in one model with strong string-coupling - non-perturbative - in another. 

After the second superstring revolution occurred, Joseph Polchinski realized that D-branes, which he discovered six years earlier, correspond to stringy versions of the $p$-branes known in supergravity theories. String theory perturbation didn't restrict these $p$-branes and thanks to supersymmetry, supergravity $p$-branes were understood to play an important
role in our understanding of string theory. Armed with this new nonperturbative tool, Edward Witten and many others could show all of the perturbative string theories as descriptions of different states in a single theory that Witten named M-theory \cite{witten2}, \cite{duff}. Furthermore, he argued that M-theory's long wavelength limit, i.e. when the quantum wavelength associated to objects in the theory appear much larger than the size of the 11th dimension,
is described by 11-dimensional supergravity. Certain extended
objects, the M2 and M5-branes, which arise in the context D=11 supergravity,
but whose relationship with the ten-dimensional branes was unclear, were then
understood to play an important role in M-theory.
 It is a general feature that in the presence of branes, the flatspace supersymmetry alegbras are modified beyond the super Poincar\'e algebra by including terms which contain topological charges of the branes.
 For individual brane configurations these take the form,
\bea
\frac{1}{p!}(C \Gamma_{\mu_1 \dots \mu_p})_{\alpha \beta}Z^{\mu_1 \dots \mu_p} \ ,
\ee
where $C$ is the charge conjugation matrix, $X^{\mu}$ are spacetime coordinates and $\Gamma_{\mu_1 \dots \mu_p}$ an antisymmetric combination of $p$ Dirac Gamma matrices in a particular supergravity theory. For example in $D=11$ supergravity, the theory contains the M2 and M5-Brane which have the 2-form $Z_{\mu \nu}$ and 5-form $Z_{\mu_1 \dots \mu_5}$ charges respectively and the SUSY algebra therefore takes the form,
\bea
\{Q_{\alpha}, Q_{\beta}\} = (C\Gamma^{\mu})_{\alpha \beta}P_{\mu} + \frac{1}{2!}(C\Gamma_{\mu_1 \mu_2})_{\alpha \beta}Z^{\mu_1 \mu_2} + \frac{1}{5!}(C\Gamma_{\mu_1 \dots \mu_5})_{\alpha \beta}Z^{\mu_1 \dots \mu_5}
\ee
Therefore, supergravity comes full circle and uses a common framework in understanding features of string theories, M-theory, and their compactifications to lower spacetime dimensions.


\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=250pt]{miiasugra.png}
	\end{center}
  \caption{Compactification/Low energy limit}
  \label{fig:msugraiia}
\end{figure}

In string theory, black holes can be constructed as systems of intersecting branes. This was
found for instance in \cite{townsend}, where black hole solutions of five dimensional ungauged supergravity
can be uplifted to solutions of D = 11 supergravity which correspond to systems of intersecting
branes. Black holes in D = 5 gauged supergravity can also be uplifted to solutions in type IIB
supergravity \cite{chamblin}. We also mention that when uplifted to higher dimensions, the supersymmetric
black ring becomes a black supertube \cite{elvang}, and is reproduced in M-theory as a system of
intersecting M2- and M5-branes.

\section{Summary of Research}
It has been known for some time that the black hole solutions of 4-dimensional theories with physical matter
couplings have event horizons with spherical topology. As a result black holes have a spherical shape and they describe
the gravitational field of stars after they have undergone gravitational collapse. In addition in four dimensions, several black hole uniqueness theorems have been shown which essentially state that black holes in four dimensions are determined by their mass, angular momentum and charge. In recent years most of the proposed  unified theories of all four fundamental forces of nature, like string theory, are defined in more than four dimensions. Many such theories have black hole solutions. As a result, the shape as well as the uniqueness theorems
for blacks need re-examining. It is known that in five dimensions that apart from the spherical black holes, there are solutions
for which the event horizon has  ring topology. Moreover,
there are known examples of five-dimensional black objects with non-spherical
horizon topology, which nevertheless have the same asymptotic charges as 
the solutions with spherical horizon cross sections. As a result, the uniqueness theorems of black holes in four do not extend to five and possibly higher dimensions.

As we have explained above, supergravities are gravitational theories coupled to appropriate
matter, including fermionic fields, and describe the dynamics of string theory at low energies. One way to investigate the geometry of black holes is to assume that
the solutions have a sufficiently large number of commuting rotational isometries. 
However, in this thesis, we shall instead consider supersymmetric black holes.
This means  that in addition to field equations the black holes solve a set of first order non-linear
differential equations which arise from the vanishing of the supersymmetry transformations of the fermions
of supergravity theories. These are the so-called Killing spinor equations (KSEs).
The understanding of supersymmetric black holes that it is proposed is facilitated
by the recent progress that has been made towards understanding the geometry of all supersymmetric backgrounds of supergravity theories. In particular, we shall exploit the fact that an extremal black hole has a well-defined near-horizon limit which solves the same field equations as the full black hole solution. Classifying near-horizon geometries is important as it reveals the geometry and hence the topology and isometries of the horizon of the full black hole solution. It also becomes simpler to solve as we can reduce it to $(D-2)$-dimensional problem on a compact spatial manifold. The classification of near-horizon geometries in a particular theory provides important information about which black hole solutions are possible.

The enhancement of supersymmetry near to brane and black hole horizons has been known
for some time. In the context of branes, many solutions are known which exhibit supersymmetry
enhancement near to the brane. For example, the geometry of D3-branes  doubles its supersymmetry to become the maximally supersymmetric $AdS_5 \times S^5$
solution \cite{gwgpkt, Schwarz:1983qr}. This phenomenon played a crucial role in the early development of the
ADS/CFT correspondence \cite{maldacena}. Black hole solutions are also known to exhibit
supersymmetry enhancement; for example in the case of the five-dimensional BMPV black hole \cite{BMPV1, Chamseddine:1996pi, Chamseddine:1999qs}. Further recent interest in the geometry of black hole horizons has arisen in the context of
the Bondi-Metzner-Sachs (BMS)-type symmetries associated with black holes, following 
\cite{Hawking:2016msc, Hawking:2016sgy, Averin:2016ybl, Donnay:2015abr}.
In particular, the analysis of the asymptotic symmetry group of Killing horizons was undertaken in
\cite{Akhmedov:2017ftb}. In that case, an infinite dimensional symmetry group is obtained,
analogous to the BMS symmetry group of asymptotically flat solutions. 

Another important observation in the study of black holes is the attractor mechanism.
This states that the entropy is obtained by extremizing an entropy function which depends only on
the near-horizon parameters and conserved charges, and if this admits a unique extremum then the entropy is independent of the asymptotic values of the moduli.
In the case of 4-dimensional solutions the analysis of \cite{astef} implies that if
the solution admits $SO(2,1) \times U(1)$ symmetry, and the horizon has 
spherical topology, then such a mechanism holds. 
In $D=4, 5$ it is an observation that all known asymptotically flat black hole solutions exhibit attractor mechanism behaviour.
However, in higher dimensions, it is unclear if an attractor mechanism holds. In particular, a generalization of the analysis
of \cite{astef} to five dimensions would require the existence of
a $SO(2,1) \times U(1)^2$ symmetry, as well as an understanding of the horizon topology. Near horizon geometries of asymptotically $AdS_5$ 
supersymmetric black holes admitting a $SO(2,1) \times U(1)^2$ symmetry have been 
classified in \cite{Kunduri:2006ek, Kunduri:2007qy}. It remains to be determined
if all supersymmetric near-horizon geometries fall into this class. 

We shall consider the following conjecture concerning the properties
of supersymmetric regular near-horizon geometries, for which all fields are smooth
and the spatial cross section of the event horizon, ${\cal{S}}$, is smooth and compact 
without boundary:
\vskip 0.3cm
{\it Theorem:} The Horizon Conjecture
\begin{itemize}
	\item the number of Killing spinors $N$, $N\not=0$,  of Killing horizons in supergravity is given by
	\begin{eqnarray}
	N = 2N_{-} + \mathrm{Index}(D_{E})~,
	\label{indexcon}
	\label{index}
	\end{eqnarray}
	where $N_{-}\in {\mathbb{N}}_{>0}$ and $D_{E}$ is a Dirac operator twisted by a vector bundle $E$, defined on the spatial horizon section $\mathcal{S}$, which depends on the gauge symmetries of the supergravity theory in question,
	\item that horizons with non-trivial fluxes and $N_{-} \neq 0$ admit an $\mathfrak{sl}(2,{\mathbb{R}})$ symmetry subalgebra.
\end{itemize} 

One simple motivational example of (super)symmetry enhancement which we will consider in the next chapter is the $\mathbb{R} \times SO(3)$ isometry group of the Reissner-Nordstr\"om black hole which in the extremal near-horizon limit enhances to $SL(2, \mathbb{R}) × SO(3)$ with near-horizon geometry $AdS_2 \times S^2$. In addition, viewing the extreme Reissner-Nordstrom black hole as a solution of the ${\cal{N}} = 2, d = 4$ minimal supergravity, the $N = 4$ supersymmetry of the solution also
enhances to $N = 8$ near the horizon.

The main focus of this thesis is to prove the horizon conjecture for supersymmetric black hole horizons of IIA, massive IIA and $D=5$ (gauged and ungauged) supergravity with vector multiplets. In particular, the first part of
the horizon conjecture as applied to these theories will establish that
there is supersymmetry enhancement, which gives rise to symmetry enhancement
in the form of the $\mathfrak{sl}(2,{\mathbb{R}})$ symmetry, as mentioned
in the second part of the horizon conjecture. Such symmetry enhancement
also produces additional conditions on the geometry of the solution.
 The methodology used to investigate these problems involves techniques in differential geometry, differential equations on compact manifolds, and requires some knowledge on general relativity and supergravity. Algebraic and differential topology are also essential in the analysis. 

The proofs that we establish in this thesis for (super)symmetry enhancement rely on establishing Lichnerowicz-type theorems and an index theory argument. A similar proof has been given for supergravity horizons in $D=11$, IIB, $D=5$ minimal gauged and $D=4$ gauged \cite{11index, iibindex, 5dindex, 4dindex}. 
We shall also prove that the near-horizon geometries admit a $\mathfrak{sl}(2,\mathbb{R})$
symmetry algebra. In general we find that the orbits of the generators of $\mathfrak{sl}(2,\mathbb{R})$ are
3-dimensional, though in some special cases they are 2-dimensional. In these special cases,
the geometry is a warped product $AdS_2 \times_w {\cal{S}}$.
The properties of $AdS_2$ and their relationship to black hole entropy
have been examined in \cite{strominger, sen}.
Our results, together with those of our previous calculations, implies 
that the $\mathfrak{sl}(2,\mathbb{R})$ symmetry is a universal property of supersymmetric black holes.

The new Lichnerowicz type theorems established in this thesis are of interest
because they have certain free parameters appearing in the definition
of various connections and Dirac operators on ${\cal{S}}$. Such freedom
to construct more general types of Dirac operators in this way is related to
the fact that the minimal set of Killing spinor equations consists not
only of parallel transport conditions on the spinors, but also 
certain algebraic conditions. These algebraic conditions do
not arise in the case of $D=11$ supergravity. Remarkably, the Lichnerowicz type
theorems imply not only the parallel transport conditions, but also
the algebraic ones as well. The solution of the KSEs is essential to the investigation of geometries
of supersymmetric horizons. We show that the enhancement of the supersymmetry
produces a corresponding symmetry enhancement, and describe the resulting conditions
on the geometry. The only
assumptions we make are that the fields are smooth (or at least $C^2$ differentiable)
and the spatial horizon section ${\cal S}$ is compact without boundary.\footnote{This
is an assumption which can be relaxed. To extend the proof to horizons with non
compact ${\cal S}$, one has to impose boundary conditions on the fields.}

\subsection{Plan of Thesis}

In {\bf Chapter 2}, we describe the properties of Killing Horizons and introduce Gaussian Null Coordinates (GNC), and we explicitly state important examples in $D=4$ in these coordinates, paying particular attention to extremal horizons. We also introduce the Near-Horizon Limit (NHL) and give explicit examples for the extremal Reissner-Nordstr\"om, Kerr and Kerr-Newman to demonstrate the symmetry enhancement with the ${\mathfrak{sl}}(2,{\mathbb{R}})$ lie algebra of the Killing vectors. We then give an overview of the curvature of the ear-horizon geometry, field strengths in the near horizon limit, the supercovariant derivative, the maximum principle and the classical Lichnerowicz theorem.

In {\bf Chapter 3}, we summarize the various types of supergravity theories which we will consider in this thesis. We begin with an overview of $D=11$ supergravity stating the action, the supersymmetry variations and the field equations, which we will do for every supergravity theory that we consider. We also give the details for dimensional reduction on ${\cal M}_{10} \times S^1$ which gives $D=10$ IIA supergravity on ${\cal{M}}_{10}$. We also give the Romans Massive IIA which give extra terms that depend on the mass parameter $m$. Next we consider the dimensional reduction of $D=11$ supergravity on ${\cal M}_{5} \times CY_3$ and give the details for $D=5$ (ungauged) supergravity coupled to an arbitrary number of vector multiplets on ${\cal M}_{5}$ and the Very Special Geometry associated with the Calabi Yau manifold. Finally, we summarize the details for $D=5$ gauged supergravity with vector multiplets, which give extra terms that depend 
on the gauging parameter $\chi$.

We begin the {\it general analysis} of supersymmetric near-horizon geometries by solving the KSEs along the lightcone direction, identifying the redundant conditions and stating the independent KSEs, field equations and bianchi identities given as the restriction on the spatial horizon section. By an application of the Hopf maximum principle, we establish generalised Lichnerowicz theorems relating the zero modes of the horizon Dirac equation with the KSEs. Using the index theorem, we then establish the enhancement of supersymmetry and show that the number of supersymmetries must double. Finally by identifying the isometries generated by the Killing vectors of the the Killing spinor bilinear with the solution along the light cone, we show the enhancement of symmetry with the $\mathfrak{sl}(2,\mathbb{R})$ lie subalgebra.

In {\bf Chapter 4} we give the details of the {\it general analysis} in proving the horizon conjecture for IIA supergravity. In particular we give the near horizon fields, the horizon bianchi identities and field equations. We then solve the KSEs of IIA supergravity along the lightcone and identify the independent conditions. We then prove the supersymmetry enhancement by identifying the horizon Dirac equation, establishing the Lichnerowizc theorems and using the index theory. We also give the details of the $\mathfrak{sl}(2,\mathbb{R})$ symmetry enhancement for IIA horizons. In {\bf Chapter 5} we repeat the {\it general analysis} with the addition of the mass parameter $m$.

In {\bf Chapter 6} we give a brief introduction into the near-horizon geometry of the BMPV and black ring solution in Gaussian Null Coordinates, and explicitly show how the symmetry enhancement in the near-horizon limit produces Killing vectors which satisfy the $\mathfrak{sl}(2,\mathbb{R})$ Lie algebra. We then repeat the same {\it general analysis} as previous chapters, for $D=5$ supergravity (gauged and ungauged) with vector mulitplets. We also hightlight differences in the gauged and ungauged theories, particularly in counting the number of supersymmetries and the conditions on the geometry of $\cal{S}$.

In the appendices, we give the calculations required for the analysis of the various supergravity theories we have considered. In particular, {\bf Appendix A} gives the details for the derivation of Gaussian Null Coordinates and other regular coordinate systems. {\bf Appendix B} we explicitly give the expressions used in computing the spin connection, Riemann tensor and Ricci tensor. {\bf Appendix C} gives the calculations for IIA supergravity, we first give the integrability conditions from the KSEs which give rise to the field equations. We also give a derivation of the Dilaton field equation which is implied by the other field equations. We then give the details in establishing the conditions that we get from the solution along the lightcone in terms of the independent KSEs. We also give a proof of the Lichneorwicz principle using a maximum principle by calculating the Laplacian of the norm of the spinors. We also give an alternative derivation using a partial integration argument. In {\bf Appendix D} and {\bf Appendix E}, we repeat these details for Massive IIA, $D=5$ ungauged and gauged supergravity. Finally in {\bf Appendix F} we give the generic calculations that are required for the analysis of the $\mathfrak{sl}(2,\mathbb{R})$ symmetry and spinor bilinears.

\newpage

\section{Statement of Originality}

I hereby declare that except where specific reference is made to the work of others,
the contents of this dissertation are original and have not been submitted in whole
or in part for consideration for any other degree or qualification in this, or any other university. This dissertation is my own work and contains nothing which is the outcome of work done in collaboration with others, except as specified in the text and Acknowledgements. This thesis contains fewer than 100,000 words excluding the bibliography, footnotes, tables and equations.

\section{Publications}
  U.~Kayani, G.~Papadopoulos, J.~Gutowski, and U.~Gran,
``Dynamical symmetry enhancement near IIA horizons,''
JHEP {\bf 1506}, 139 (2015)
doi:10.1007/JHEP06(2015)139,

%%CITATION = doi:10.1007/JHEP06(2015)139;%%
U.~Kayani, G.~Papadopoulos, J.~Gutowski, and U.~Gran,
``Dynamical symmetry enhancement near massive IIA horizons,''
Class.\ Quant.\ Grav.\  {\bf 32}, no. 23, 235004 (2015)
doi:10.1088/0264-9381/32/23/235004
  
U.~Kayani,``Symmetry enhancement of extremal horizons in D  =  5 supergravity,''
%``Symmetry enhancement of extremal horizons in D  =  5 supergravity,''
Class.\ Quant.\ Grav.\  {\bf 35}, no. 12, 125013 (2018)
doi:10.1088/1361-6382/aac30c
%%CITATION = doi:10.1088/1361-6382/aac30c;%%

==> lich/lich.tex <==
\chapter{Lichnerowicz and maximum principle}

We give a reminder of the classical Lichnerozicz theorem and the Maximum principle, which are crucial in establishing the results of (super)symmetry enhancement.

\section{The (classical) Lichnerowicz Theorem}

On any spin compact manifold $N$, one can show the equality
\bea
\int_N \langle \Gamma^i \nabla_i \epsilon, \Gamma^j \nabla_j \epsilon \rangle=  \int_N \langle  \nabla_i \epsilon ,  \nabla^i \epsilon \rangle+\int_N {R\over 4} \langle \epsilon , \epsilon \rangle~,
\ee

\bea
{\cal{I}} &=& \int_{{\cal{M}}} \big ( \parallel \nabla \epsilon\parallel^2-\parallel{\cal D} \epsilon \parallel^2\big)~,
\ee

\bea
{\cal{I}} = \int_{{\cal{M}}} \langle \nabla_i \epsilon ,\nabla^i \epsilon \rangle
- \langle \Gamma^i \nabla_i \epsilon ,
 \Gamma^j \nabla_j \epsilon \rangle~.
\ee

\bea
{\cal{I}} = \int_{{\cal{M}}} -\nabla_{i}\langle \epsilon, \Gamma^{i j}\nabla_{j}\epsilon \rangle + \int_{{\cal{M}}} \langle \epsilon, \Gamma^{i j}\nabla_i \nabla_j \epsilon\rangle
\ee
where $\nabla$ is the Levi-Civita connection, $\langle \cdot, \cdot\rangle$ is the Dirac inner product and $R$ is the Ricci scalar. Clearly if $R>0$, the Dirac operator has no zero modes. Moreover, if $R=0$, then the zero modes of the Dirac operator are parallel with respect to the Levi-Civita connection.

Alternatively. if $\epsilon$ satisfies the Dirac equation $\Gamma^{i}\nabla_{i}\epsilon = 0$, then
\bea
\nabla^{i}\nabla_{i}||\epsilon||^2 = \frac{1}{2}R||\epsilon||^2 + 2\langle \nabla_{i}\epsilon, \nabla^{i}\epsilon \rangle
\ee

To proceed, we compute the Laplacian
\bea
\nabla^i \nabla_i ||\epsilon||^2 = 2\langle\epsilon ,\nabla^i \nabla_i\epsilon\rangle + 2 \langle\nabla^i \epsilon, \nabla_i \epsilon\rangle \ .
\ee
To evaluate this expression note that
\bea
\nabla^i \nabla_i \epsilon &=& \Gamma^{i}\nabla_{i}(\Gamma^{j}\nabla_j \epsilon) -\Gamma^{i j}\nabla_i \nabla_j \epsilon
\nonumber \\
&=& \Gamma^{i}\nabla_{i}(\Gamma^{j}\nabla_j \epsilon) + \frac{1}{4}R\epsilon
\nonumber \\
&=&  \frac{1}{4}\tilde{R} \epsilon \ .
\ee

\section{The maximum principle}
\begin{comment}
\section{Vacuum}
\bea
S = \int d^{D}x \sqrt{-g} R
\ee
with $R_{\mu \nu} = 0$
\bea
\label{vGSE}
{\cal D}_{\mu}\epsilon = \nabla_{\mu}\epsilon = 0
\ee
\bea
[{\cal D}_{\mu}, {\cal D}_{\nu}]\epsilon = [\nabla_{\mu}, \nabla_{\nu}]\epsilon = \frac{1}{4}R_{\mu \nu, \rho \sigma}\Gamma^{\rho \sigma}
\ee
\bea
\Gamma^{\nu}[{\cal D}_{\mu}, {\cal D}_{\nu}]\epsilon = \frac{1}{4}\Gamma^{\nu} R_{\mu \nu, \rho \sigma} \Gamma^{\rho \sigma} = \frac{1}{4}R_{\mu \nu, \rho \sigma}(\Gamma^{\nu \rho \sigma} + 2g^{\nu [ \rho}\Gamma^{\sigma]}) = -\frac{1}{2}R_{\mu \sigma} \Gamma^{\sigma}
\ee
\bea
\nabla_{\mu} \epsilon &=& \partial_{\mu} \epsilon + \frac{1}{4}\Omega_{\mu, \nu \rho}\Gamma^{\nu \rho} \epsilon 
\nonumber \\
&=& \partial_{\mu} \epsilon + \frac{1}{4}(2\Omega_{\mu, +i}\Gamma^{+i} + 2\Omega_{\mu, -i}\Gamma^{-i} + 2\Omega_{\mu, +-}\Gamma^{+-} + \Omega_{\mu, jk}\Gamma^{jk}) \epsilon 
\nonumber \\
&=& \partial_{\mu} \epsilon + \frac{1}{2}\Omega_{\mu, +i}\Gamma^{+i}\epsilon + \frac{1}{2}\Omega_{\mu, -i}\Gamma^{-i}\epsilon + \frac{1}{2}\Omega_{\mu, +-}\Gamma^{+-}\epsilon + \frac{1}{4}\Omega_{\mu, jk}\Gamma^{jk}\epsilon
\nonumber \\
\ee
We can expand along the $\mu = +, -, i$ directions to obtain,
\bea
\nabla_+ \epsilon &=& \partial_+ \epsilon + \frac{1}{4}r^2(\Delta h_i - \partial_i \Delta)\Gamma^{+i}\epsilon - \frac{1}{4}h_i\Gamma^{-i}\epsilon - \frac{1}{2}r\Delta\Gamma^{+-}\epsilon - \frac{1}{8}r(dh)_{ij}\Gamma^{ij}\epsilon
\nonumber \\
\ee
\bea
\nabla_{-} \epsilon = \partial_{-} \epsilon - \frac{1}{4}h_i \Gamma^{+i}\epsilon
\ee
\bea
\nabla_{i} \epsilon &=& \partial_i \epsilon - \frac{1}{4}r(dh)_{ij}\Gamma^{+j}\epsilon + \frac{1}{4}h_i \Gamma^{+-}\epsilon + \frac{1}{4}\tilde{\Omega}_{i,jk}\Gamma^{jk}\epsilon 
\nonumber \\
&=& \nabla_{i}\epsilon - r\partial_{r} \epsilon h_i - \frac{1}{4}r(dh)_{ij}\Gamma^{+j}\epsilon + \frac{1}{4}h_i \Gamma^{+-}\epsilon
\ee
The description of the metric near extreme Killing horizons as expressed in Gaussian null coordinates can be written as,
\be
ds^2 &=&2 \bbe^+ \bbe^- + \delta_{ij} \bbe^i \bbe^j~,
\ee
where we have introduced the frame
\be
\label{basis1}
\bbe^+ = du, \qquad \bbe^- = dr + rh -{1 \over 2} r^2 \Delta du, \qquad \bbe^i = e^i_I dy^I~,
\ee
and the dependence on the coordinates $u$ and $r$ is explicitly given. The spatial horizon section ${\cal S}$, is the co-dimension 2 submanifold given by the equation  $r=u=0$, i.e.~all these
components of the fields depend only on the coordinates of ${\cal S}$.
We can evaluate the Einstein field equation along the lightcone. This gives
\bea
\label{veq1}
{1 \over 2} \tn^i h_i -\Delta -{1 \over 2}h^2
&=& 0~,
\ee
and
\bea
\label{veq2}
{\tilde{R}}_{ij} &=& -\tn_{(i} h_{j)}
+{1 \over 2} h_i h_j 
\ee
where $\tilde \nabla$ is the Levi-Civita connection of the metric on ${\cal S}$. Note also that the $++$ and $+i$ components of the
Einstein equation, which are
\bea
\label{veq3}
{1 \over 2} \tn^i \tn_i \Delta -{3 \over 2} h^i \tn_i \Delta-{1 \over 2} \Delta \tn^i h_i
+ \Delta h^2 +{1 \over 4} dh_{ij} dh^{ij} = 0
\ee
and
\bea
\label{veq4}
{1 \over 2} \tn^j dh_{ij}-dh_{ij} h^j - \tn_i \Delta + \Delta h_i = 0
\ee
are implied by ({\ref{veq1}}), ({\ref{veq2}}) as shown in the previous section. We can integrate (\ref{veq1}) over the horizon section $\cal{S}$ to find
\bea
\int_{\cal{S}} \bigg(\Delta +{1 \over 2}h^2\bigg) = 0,
\ee
Assuming $\Delta \geq 0$ we have $\Delta = 0, h=0$ thus the horizon section is ${\cal{S}} = T^{d-2}$ and the near-horizon geometry is locally isometric to $\R^{1,d-1}$. Here we don't need to consider the supersymmetry variations to classify the geometry, since the bosonic field equations are enough to establish this. Nonetheless, we can find the conditions required for such a solution to exist as the steps will be similar when we consider the near-horizon geometries of the various supergravity theories considered in this thesis. We can first integrate along the two lightcone directions, i.e.~we integrate the KSEs
along the $u$ and $r$ coordinates. To do this, we decompose $\epsilon$ as
\bea
\e=\e_++\e_-~,
\label{vksp1}
\ee
 where $\Gamma_\pm\epsilon_\pm=0$, and find that
\bea\label{vlightconesol}
\e_+=\phi_+(u,y)~,~~~\e_-=\phi_- + \frac{1}{4} r \Gamma_- h_{i}\Gamma^{i} \phi_+~,
\ee
and
\bea
\phi_-=\eta_-~,~~~\phi_+=\eta_+ + \frac{1}{4} u \Gamma_+ h_{i}\Gamma^{i} \eta_-~,
\ee
and $\eta_\pm$ depend only on the coordinates of the spatial horizon section ${\cal S}$. As spinors on ${\cal S}$, $\eta_\pm$ are sections of the $Spin(D-2)$ bundle on ${\cal S}$
associated with the appropriate representation.  Equivalently, the $Spin(D-1,1)$ bundle $S$ on the spacetime when restricted to ${\cal S}$ decomposes
as $S=S_-\oplus S_+$ according to the lightcone projections $\Gamma_\pm$. Although $S_\pm$ are distinguished by the lightcone chirality, they are isomorphic
as $Spin(D-2)$ bundles over ${\cal S}$. We shall use this in the counting of supersymmetries horizons.

Substituting the solution of the KSEs along the lightcone directions (\ref{vlightconesol})  back into the gravitino KSE (\ref{vGSE}) and appropriately expanding in the $r,u$ coordinates, we find that
for  the $\mu = \pm$ components, one obtains  the additional conditions
\bea
\label{vint1}
&&\bigg({1\over2}\Delta - {1\over8}(dh)_{ij}\Gamma^{ij} +  {1\over 8}h^2 \bigg)\phi_{+} = 0
\ee
\bea
\label{vint2}
&&\bigg(\frac{1}{4}\Delta h_i \Gamma^{i} - \frac{1}{4}\partial_{i}\Delta \Gamma^{i}  -\frac{1}{32}(dh)_{ij}h_{k}\Gamma^{i j k} + \frac{1}{32}(dh)_{i j}h^{j}\Gamma^{i} \bigg) \phi_{+} = 0,
\nonumber \\
\ee
\bea
\label{vint3}
&&\bigg(-\frac{1}{2}\Delta - \frac{1}{8}(dh)_{ij}\Gamma^{ij} - {1\over 8} h^2 \bigg)\phi_{-} = 0 \ .
\ee
Where $\Theta = \frac{1}{4}h_{i}\Gamma^{i}$. Similarly the $\mu=i$ component gives
\bea
\label{vint4}
&&\tilde \nabla_i \phi_\pm\mp {1\over 4} h_i \phi_\pm = 0
\ee
and
\bea
\label{vint5}
\tilde \nabla_i \tau_{+} -\frac{3}{4} h_i\tau_{+} -\frac{1}{4}(dh)_{ij}\Gamma^{j} \phi_{+} = 0
\ee
where we have set
\bea
\label{iiaint6}
\tau_{+} = \Theta \phi_{+} \ .
\ee
All the conditions above can be viewed as integrability conditions along the lightcone and mixed lightcone and ${\cal S}$ directions. 

The substitution of the  spinor (\ref{vksp1}) into the KSEs produces a large number of additional conditions.  These can be seen
either as integrability conditions along the lightcone directions, as well as integrability conditions along the mixed lightcone and
${\cal S}$ directions, or as KSEs along ${\cal S}$. A detailed analysis, of the formulae obtained reveals
that the independent KSEs are those that are obtained from the naive restriction of the KSE to ${\cal S}$.  In particular,
the independent KSEs are
\bea
\label{vcovr}
\nabla_{i}^{(\pm)}\eta_{\pm}  = 0~,
\ee
where
\bea
\nabla_{i}^{(\pm)}&=& \nabla_{i} \mp \frac{1}{4}h_{i}~,
\ee
with
$\nabla^{(\pm)}$ arise from the supercovariant connection as restricted to ${\cal S}$ .
One can also show that if $\eta_{-}$ solves $(\ref{vcovr})$ then,
\bea
\eta_+ = \Gamma_{+}\Theta \eta_{-}~,
\label{vepfem}
\ee
 also solves $(\ref{vcovr})$. 

To prove that such horizons always admit an even number of supersymmetries, one has to prove that there are as many $\eta_+$ Killing spinors as there are $\eta_-$ Killing spinors,
i.e.~that the $\eta_+$ and $\eta_-$ Killing spinors come in pairs. For the vacuum case this is not possible since we have $\Theta = 0$ from the analysis of (\ref{veq1}) or the integrability condition (\ref{vint1}) as we shall show in what follows.
For this, we shall identify the Killing spinors with the zero modes of  Dirac-like operators
which depend on the fluxes and then use the index theorem to count their modes.

We define  horizon Dirac operators associated with the supercovariant derivatives following from the gravitino KSE as
\bea
{\cal D}^{(\pm)} \equiv \Gamma^{i}\nabla_{i}^{(\pm)} = \Gamma^{i}\nabla_{i}  \mp\frac{1}{4}h_{i}\Gamma^{i}~,
\ee

First let us establish that the $\eta_+$ Killing spinors can be identified with the zero modes of a ${\cal D}^{(+)}$.  It is straightforward to see
that if $\eta_+$ is a Killing spinor, then $\eta_+$ is a zero mode of ${\cal D}^{(+)}$. So it remains to demonstrate the converse.
For this assume that $\eta_+$ is a zero mode of ${\cal D}^{(+)}$, i.e.~${\cal D}^{(+)}\eta_+=0$, one can then establish the equality
\bea
{\nabla}^{i}{\nabla}_{i}\parallel\eta_+\parallel^2 - h^i {\nabla}_{i}\parallel\eta_+\parallel^2 = 2\parallel{\nabla^{(+)}}\eta_{+}\parallel^2,
\label{vmaxprin}
\ee
It is clear that if the last term on the right-hand-side of the above identity is positive semi-definite, then one can apply the maximum principle on $\parallel\eta_+\parallel^2$
as the fields are assumed to be smooth, and ${\cal S}$ compact. The maximum principle implies that $\eta_+$ are Killing spinors and $\parallel\eta_+\parallel=\mathrm{const}$. 
To summarize we have established that,
\bea
\nabla_{i}^{(+)}\eta_+=0~,\Longleftrightarrow~ {\cal D}^{(+)}\eta_+=0~.
\ee
Moreover $\parallel\eta_+\parallel^2$ is constant on ${\cal S}$.

Next we shall establish that the $\eta_-$ Killing spinors can also be identified with the zero modes of a modified horizon Dirac operator ${\cal D}^{(-)}$.
It is clear that all Killing spinors $\eta_-$ are zero modes of ${\cal D}^{(-)}$. To prove the converse,
suppose that $\eta_-$ satisfies ${\cal D}^{(-)} \eta_-=0$.
The proof proceeds by calculating the Laplacian of $\parallel \eta_-
\parallel^2$. One can then establish the formula
\bea
\label{vl2b}
{\nabla}^{i} \big( \nabla_{i}\parallel \eta_- \parallel^2 + \parallel \eta_- \parallel^2 h_{i} \big)
= 2 \parallel{\nabla^{(-)}}\eta_{-}\parallel^2~,
\ee
The last term on the RHS of ({\ref{vl2b}}) is negative semi-definite and on integrating ({\ref{vl2b}}) over
${\cal{S}}$ and assuming that ${\cal{S}}$ is compact and without boundary, one finds that ${\nabla^{(-)}}\eta_{-}=0$.
Therefore, we have shown that
\bea
\nabla_{i}^{(-)}\eta_-=0~,\Longleftrightarrow~ {\cal D}^{(-)}\eta_-=0~ \ .
\ee
This concludes the relationship between Killing spinors and zero modes of modified horizon Dirac operators.

From the integrability condition (\ref{vint1}) one can also show
\bea
\bigg({1\over2}\Delta +  {1\over 8}h^2 \bigg)\parallel\eta_+\parallel^2 = 0,
\ee
since $\parallel\eta_+\parallel^2$ is constant, we have find $h=0, \Delta =0$ which is consistent with the result we obtained from the decomposition of the vacuum einstein equation (\ref{veq1}).

In the investigation of the integrability conditions, one can show in the analysis of the independent conditions that if $\eta_-$ is a Killing spinor, then
$\eta_+ = \Gamma_+ \Theta \eta_-$ is also a Killing spinor. Since we know that the $\eta_+$ and $\eta_-$ Killing spinors
appear in pairs, the formula (\ref{vepfem}) provides a way to construct the $\eta_+$ Killing spinors from the $\eta_-$ ones.
However, this is only the case provided that $\eta_+=\Gamma_+ \Theta \eta_-\not=0$. For the vacuum case, this does not hold since $h=0$ implies $\Theta = 0$.
\end{comment}
